A General Theory for Client Sampling in Federated Learning

While client sampling is a central operation of current state-of-the-art federated learning (FL) approaches, the impact of this procedure on the convergence and speed of FL remains under-investigated. In this work, we provide a general theoretical framework to quantify the impact of a client sampling scheme and of the clients heterogeneity on the federated optimization. First, we provide a unified theoretical ground for previously reported sampling schemes experimental results on the relationship between FL convergence and the variance of the aggregation weights. Second, we prove for the first time that the quality of FL convergence is also impacted by the resulting covariance between aggregation weights. Our theory is general, and is here applied to Multinomial Distribution (MD) and Uniform sampling, two default unbiased client sampling schemes of FL, and demonstrated through a series of experiments in non-iid and unbalanced scenarios. Our results suggest that MD sampling should be used as default sampling scheme, due to the resilience to the changes in data ratio during the learning process, while Uniform sampling is superior only in the special case when clients have the same amount of data.

==> tex/abbreviations.tex <==
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\eqnref}[1]{Eq.~(\ref{#1})}

\newcommand{\tbc}[0]{\textbf{> > > TO BE CHECKED < < <}}
\newcommand{\tbm}[0]{\textbf{> > > TO BE MODIFIED < < <}}
\newcommand{\tbe}[0]{\textbf{> > > TO BE EXPANDED < < <}}

\newcommand{\cf}[0]{\textit{cf. }}
\newcommand{\eg}[0]{\textit{e.g., }}
\newcommand{\ibid}[0]{\textit{ibid.}}
\newcommand{\ie}[0]{\textit{i.e.,}}

\newcommand{\suppmat}[0]{\hyperref[sec:supmat]{\textit{Supplementary Material}} }
\newcommand{\asuppmat}[0]{\hyperref[sec:supmat]{\textit{Sup. Mat.}} }


==> tex/clustered_sampling.tex <==
\section{Clustered sampling}\label{app:clustered_sampling}


\begin{lemma}[One server iteration progress for Clustered Sampling]\label{lem:inequality_update_clustered}
	We consider a client sampling satisfying Definition \ref{def:sampling} and with aggregation weight covariance satisfying $\COV{\omega_i(S_t)}{\omega_j(S_t)} = \alpha p_i p_j$. Then, FedAvg updates satisfy:
	
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} \inner{\sum_{i, k}p_i \EE{t}{\nabla \Lcal_i(y_{i,k}^t)} }{\theta^t - \theta^*} \nonumber\\
	&+ \eta_g^2 \sum_{i}\frac{1}{m}p_i \EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 } 
	 + \eta_g^2 (1- \frac{1}{m}) \EE{t}{\norm{\sum_i p_i (\theta_i^{t+1} - \theta^t)}^2}.
	\end{align}	
\end{lemma}

\begin{proof}
	We note that the proof for Lemma \ref{lem:inequality_update_clustered} is similar to the one of Lemma \ref{lem:equality_update_without_Jenken}. Its difference lies in the reexpression of $B$. Equation (\ref{app:eq:express_B}) still holds. However, there is no $\alpha$ enabling expression of the covariance fitting for Lemma \ref{lem:equality_update_without_Jenken}. We have:
	\begin{align}
		B 
		& = \sum_{i=1}^n\VARR{S_t}{\omega_i(S_t)}\EE{t}{\norm{\theta_i^{t+1} - \theta^t }^2 } \nonumber\\
		&+ \sum_{i, j \neq i}\COV{\omega_i(S_t)}{\omega_j(S_t)}\EE{t}{\inner{\theta_i^{t+1} - \theta^t}{\theta_j^{t+1} - \theta^t} }
		\label{app:eq:H1}
	\end{align}
		
	We have:
	\begin{align}
		\COV{\omega_i(S_t)}{\omega_j(S_t)} 
		&= \E{\omega_i(S_t)\omega_j(S_t)} - p_i p_j\\
		&= \frac{1}{m^2}\sum_{k=1}^{m}\sum_{l=1}^{m}\E{\{l_k =i\}\{l_l = i\}} - p_i p_j\\
		&= \frac{1}{m^2}\sum_{k=1}^{m}\sum_{l\neq k} r_{k, i}r_{l, i} - p_i p_j\\
		&= \frac{1}{m^2}\sum_{k=1}^{m} r_{k, i}( m p_j- r_{k, j}) - p_i p_j\\
		&= -\frac{1}{m^2}\sum_{k=1}^{m} r_{k, i}r_{k, j}
		\label{app:eq:H2}
	\end{align}
	
	Considering that $\E{\{l_k =i\}^2} = r_{k, i}$, we have with a similar reasoning:
	We have:
	\begin{align}
	\VAR{\omega_i(S_t)}
	&= \frac{1}{m^2}\sum_{k=1}^{m}\sum_{l\neq k} r_{k, i}r_{l, i} 
	+ \frac{1}{m^2}\sum_{k=1}^{m}r_{k, i}
	- p_i p_j\\
	&= -\frac{1}{m^2}\sum_{k=1}^{m} r_{k, i}^2 + \frac{1}{m} p_i
	\label{app:eq:H3}
	\end{align}
	
	We also note that:
	\begin{equation}
		\EE{t}{\norm{\sum_i r_{k, i} (\theta_i^{t+1} - \theta^t)}^2} 
		= \EE{S_t}{\sum_{i, j} r_{k,i} r_{k, j} \inner{\theta_i^{t+1} - \theta^t}{\theta_j^{t+1} - \theta^t}} 
		\label{app:eq:H4}
	\end{equation} 
	
	Substituting equation (\ref{app:eq:H2}), (\ref{app:eq:H3}), and (\ref{app:eq:H4}) in equation (\ref{app:eq:H1}), we get:
	\begin{align}
	B 
	& = \sum_{i=1}^n\VARR{S_t}{\omega_i(S_t)}\EE{t}{\norm{\theta_i^{t+1} - \theta^t }^2 } \nonumber\\
	&- \frac{1}{m^2} \sum_{i, j \neq i}\sum_{k=1}^{m} r_{k, i}r_{k, j}\EE{t}{\inner{\theta_i^{t+1} - \theta^t}{\theta_j^{t+1} - \theta^t} }\\
	& = \sum_{i=1}^n\VARR{S_t}{\omega_i(S_t)}\EE{t}{\norm{\theta_i^{t+1} - \theta^t }^2 } \nonumber\\
	&- \frac{1}{m^2} \sum_{k=1}^{m} \left[\EE{t}{\norm{\sum_i r_{k, i} (\theta_i^{t+1} - \theta^t)}^2} - \sum_{i} r_{k,i}^2 \EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2}\right]\\
	& = \frac{1}{m}\sum_{i=1}^n p_i \EE{t}{\norm{\theta_i^{t+1} - \theta^t }^2 } - \frac{1}{m^2} \sum_{k=1}^{m} \EE{t}{\norm{\sum_i r_{k, i} (\theta_i^{t+1} - \theta^t)}^2} \\
	& \le \frac{1}{m}\sum_{i=1}^n p_i \EE{t}{\norm{\theta_i^{t+1} - \theta^t }^2 } - \frac{1}{m}\EE{t}{\norm{\sum_i p_i (\theta_i^{t+1} - \theta^t)}^2}, 
	\end{align}
	where the inequality comes from using the Jensen inequality which completes the proof.
\end{proof}

\begin{theorem}[Convergence guarantees without Assumption \ref{ass:dissimilarity}]\label{theo:convergence_clustered}
	Under Assumptions \ref{ass:smoothness} to \ref{ass:unbiased}, with $\mu$ strongly convex local loss functions, with small enough local step size $\eta_l = \sqrt{m/KT}$, and for clustered sampling, we get the following convergence bound:
	\begin{align}
	\frac{1}{T+1}\sum_{t=0}^{T+1}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
	& \le \Ocal(\frac{1}{\eta_g\sqrt{m K T}}) 
	+ \Ocal(\frac{mK}{T}) 
	+ \Ocal( \sqrt{\frac{mK }{ T }} \eta_g\VAR{\sum_{i=1}^{n}\omega_i(S_t)}) \nonumber\\
	&+ \Ocal(\sqrt{\frac{mK }{ T }} \eta_g  \sum_{i=1}^{n}\delta_i \EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}).
	\label{eq:convergence_2}
	\end{align}	
\end{theorem}


\newpage











==> tex/coro_decomposition_theorem.tex <==

\subsection{Corollary \ref{cor:equality_decomposition}} \label{app:sec:cor_equa_decomposition}


We define the normalized gradients $h_i^t$ and the normalized stochastic gradient $d_i^t$ defined as:
\begin{equation}
	d_i^t = \sum_{k=0}^{K-1} g_i(y_{i, k}^t)
	\text{ and }
	h_i^t = \sum_{k=0}^{K-1} \nabla \Lcal_i (y_{i, k}^t)
\end{equation}
We also define by $\xi_i^t$ the stochastic gradient of client $i$ at optimization $t$ and defined as:
\begin{equation}
	\xi_i^t = \sum_{k=0}^{K-1} \left[ g(y_{i, k}^t) - \nabla \Lcal_i (y_{i, k}^t)\right]
	= d_i^t - h_i^t
\end{equation}
Following Assumption \ref{ass:unbiased}, we have $\E{\xi_i^t} = 0$ and $\E{{\xi_i^t}^2} \le \sigma^2$. 


\begin{proof}
    By construction, we have $\theta_i^{t+1} - \theta^t = - \sum_{k=0}^{K-1} \eta_l g_i(y_{i,k}^t) = - \eta_l d_i^t $. Hence, we can bound the local drift as :
    \begin{align}
        L_i(\theta^t)
%        = \E{\norm{\theta_i^{t+1}-\theta^t}^2}
%        \\
        = \eta_l^2 \E{\norm{d_i^t}^2}
%        \\
%        = \eta_l^2 \left[ \E{\norm{d_i^t - h_i^t}^2 }
%        +  \E{\norm{h_i^t}^2}\right]
%        \\
        = \eta_l^2 \left[ \E{\norm{\xi_i^t}^2 }
        + \E{\norm{h_i^t}^2} \right] 
%        \\
	\label{app:eq:L_i}
    \end{align}
    where the last equation comes from using Assumption \ref{ass:unbiased} which gives $\EE{\xi_i^t}{d_i^t} = h_i^t$.
    
    Similarly for the global model drift, we have:
    \begin{align}
        G(\{p_i\}, \theta^t)
%        &= \E{\norm{\sum_{i=1}^n p_i (\theta_i^{t+1}-\theta^t)}^2}
%        \\
        &= \eta_l^2 \E{\norm{\sum_{i=1}^n p_id_i^t }^2}
        \\
        &= \eta_l^2 \E{\norm{\sum_{i=1}^n p_i (d_i^t - h_i^t)}^2}
        + \eta_l^2 \E{\norm{\sum_{i=1}^n p_i h_i^t }^2}
        \\
		&= \eta_l^2 \E{\norm{\sum_{i=1}^n p_i \xi_i^t }^2}
		+ \eta_l^2 \E{\norm{\sum_{i=1}^n p_i h_i^t }^2}
		\\
		&= \eta_l^2 \left[ \sum_{i=1}^n p_i^2 \E{\norm{ \xi_i^t }^2}
		+ \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} \right],
    \end{align}
    where the last equality comes from using Assumption \ref{ass:unbiased} giving $\E{\inner{\xi_i^t}{\xi_j^t}} = \E{\xi_i^t}^T \E{\xi_j^t} =  0 $.
    
    As a result, we have:
    \begin{align}
    	\sum_{i=1}^{n} \gamma_i L_i(\theta^t) + ( 1- \alpha) G(\theta^t)
    	& = \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} 
    	+ \alpha p_i^2\right] L_i(\theta^t) + ( 1- \alpha) G(\theta^t)
    	\\
    	& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + \alpha p_i^2\right]  \left[ \E{\norm{\xi_i^t}^2 } + \E{\norm{h_i^t}^2} \right] 
    	\nonumber\\
    	& + \eta_l^2 ( 1- \alpha)  \left[ \sum_{i=1}^n p_i^2 \E{\norm{ \xi_i^t }^2}
    	+ \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} \right]
    	\\
    	& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] \E{\norm{\xi_i^t}^2 } 
    	\nonumber\\
    	& + \eta_l^2 \sum_{i=1}^{n} \gamma_i  \E{\norm{h_i^t}^2} 
    	+ \eta_l^2 ( 1- \alpha)  \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} 
    	\\
    	& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] \E{\norm{\xi_i^t}^2 } 
    	\nonumber\\
    	& + \eta_l^2 \sum_{i=1}^{n} \left[\VAR{\omega_i(S_t)} + p_i^2 \right]  \E{\norm{h_i^t}^2} 
    	+ \eta_l^2 ( 1- \alpha) \sum_{i=1}^{n}\sum_{\substack{j=1\\ j\neq i}}^{n} \E{\inner{h_i^t}{h_j^t}} 
    \end{align}
    
	where the equality comes from the unbiasedness of the SGD estimator, Assumption \ref{ass:unbiased}, and the last inequality comes from the bounded variance of the SGD estimator, Assumption \ref{ass:unbiased}.
	
	
	Let us consider the special case where clients have the same data distribution. Clients perform identical local work. Therefore, we can define $h^t \coloneqq h_i^t$. By definition, equation (\ref{eq:global_loss}), we have $\sum_{i=1}^{n}p_i = 1$ which gives $h^t = \sum_{i=1}^{n} p_i h_i^t$ which gives	
	\begin{align}
	\sum_{i=1}^{n} \gamma_i L_i(\theta^t) + ( 1- \alpha) G(\theta^t)
	& \le \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right] K \sigma^2 
	\nonumber\\
	& + \eta_l^2 \left[ \sum_{i=1}^{n} \gamma_i  + (1 - \alpha ) \right] \E{\norm{h^t}^2} 
%	+ \eta_l^2 ( 1- \alpha)  \E{\norm{\sum_{i=1}^n p_i h_i^t }^2} 
	\\& = \eta_l^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i} + p_i^2 \right] K \sigma^2 
	+ \eta_l^2 \left[ \VAR{\sum_{i=1}^{n}\omega_i}  + 1 \right] \E{\norm{h^t}^2} 
	\end{align}
	
	
\end{proof}

==> tex/different_samplings.tex <==
\section{Analysis of statistical properties of client sampling schemes} \label{sec:different_samplings}


%\begin{table}
%	\caption{Synthesis different sampling. Calculus details in Appendix \ref{app:sampling_calculus}.}
%	\label{table:sampling}
%	\centering
%	\begin{tabular}{lll}
%		\toprule
%		Sampling     
%		& $\delta_i$    
%		& $\VAR{\sum_{i=1}^{n}\omega_i(S_t)}$ \\
%		\midrule
%		MD  
%		& $= p_i$    
%		& $=0$     \\
%		
%		%		IMD   
%		%		& $= [ 1 - \gamma^* (1 - \E{|S_t|^{-1}}) ] p_i$    
%		%		& $=0$     \\
%		
%		Clustered   
%		&  $\le p_i$    
%		& $=0$     \\
%		
%		Uniform     
%		& $ = \frac{n - m}{m}( 1 + \frac{1}{n-1})p_i^2 + ( 1 - \frac{n-m}{m (n-1)}) p_i   $     
%		& $= \frac{n-m}{m (n-1)} [n \sum_{i=1}^{n}p_i^2 -1]$  \\
%		\bottomrule
%	\end{tabular}
%\end{table}

\begin{table}
	\caption{Synthesis different sampling. Calculus details in Appendix \ref{app:sampling_calculus}.}
	\label{table:sampling}
	\centering
	\begin{tabular}{lll}
		\toprule
		Sampling     
		& $\alpha$    
		& $\VAR{\sum_{i=1}^{n}\omega_i(S_t)}$ \\
		\midrule
		MD  
		& $= 1/m$    
		& $=0$     \\
		
		%		IMD   
		%		& $= [ 1 - \gamma^* (1 - \E{|S_t|^{-1}}) ] p_i$    
		%		& $=0$     \\
		
%		Clustered   
%		&  $\le p_i$    
%		& $=0$     \\
		
		Uniform     
		& $ = \frac{n - m}{m(n-1)}$     
		& $= \frac{n-m}{m (n-1)} [n \sum_{i=1}^{n}p_i^2 -1]$  \\
		
%		Poisson     
%		& $ = 0$     
%		& $= \frac{1}{m} - \sum_{i =1 }^n p_i^2 $  \\
		
%		Binomial     
%		& $ = 0$     
%		& $= \frac{n-m}{m } \sum_{i=1}^{n}p_i^2 $  \\
%		\bottomrule
	\end{tabular}
\end{table}

%\begin{table}
%	\caption{Synthesis different sampling. Calculus details in Appendix \ref{app:sampling_calculus}}
%	\label{table:sampling}
%	\centering
%	\begin{tabular}{llll}
%		\toprule
%		\multicolumn{2}{c}{Part}                   \\
%		\cmidrule(r){1-2}
%		Name     & Description     & Size ($\mu$m) \\
%		\midrule
%		Dendrite & Input terminal  & $\sim$100     \\
%		Axon     & Output terminal & $\sim$10      \\
%		Soma     & Cell body       & up to $10^6$  \\
%		\bottomrule
%	\end{tabular}
%\end{table}

%In Section \ref{sec:convergence}, we show with Theorem \ref{theo:convergence_paper} the impact a client sampling has on the convergence neighborhood radius through $\delta_i$ and $\delta$. 
In this Section, we formally express $\omega_i(S_t)$, the aggregation weight of client $i$, for MD and Uniform sampling.

\textbf{MD sampling}. We consider $l_1, ..., l_m$ to be the $m$ iid sampled clients from a multinomial distribution with support on $\{1, ..., m\}$ satisfying $\mathbb{P}(l=i) = p_i$. By definition of the federated optimization problem, equation (\ref{eq:global_loss}), we have $\sum_{i=1}^{n}p_i =1$. Hence, we can express every client aggregation weight as
\begin{equation}
\omega_i(S_t) = \frac{1}{m} \sum_{k =1 }^m \{l_k = i\}.
\label{eq:MD_aggreg_weight}
\end{equation}

\textbf{Uniform sampling}. To tackle the replacement drawback of MD sampling, Uniform sampling samples $m$ clients with identical probability without replacement. We note that for such a sampling, a client can be sampled with probability $ p(\{i \in S_t\}) = m/n$ which to satisfy Definition \ref{def:sampling} leads to:
\begin{equation}
\omega_i(S_t) 
= \{ i \in S_t\} \frac{n}{m}p_i.
\end{equation}
We note that this Uniform sampling formulation is a generalization of the Uniform sampling scheme only used for FL applications with identical client importance, i.e. $p_i = 1 / n$ \cite{SCAFFOLD, OnTheConvergence, reddi2021adaptive, DynamicFL}. We note that $\VAR{\sum_{i=1}^{n}\omega_i(S_t)} = 0$ if and only if $p_i = 1/n$ for all the clients.

We note that for both MD and Uniform sampling aggregation weight covariance there exists an $\alpha$ such that $\forall i\neq j,\  \COV{\omega_i(S_t)}{\omega_j(S_t)} = - \alpha p_i p_j$. We provide in Table \ref{table:sampling} $\alpha$ close form for these two client samplings. The calculus details to reach these close forms can be found in Appendix \ref{app:sampling_calculus}. Based on that fact, in the rest of this work, in addition of satisfying Definition \ref{def:sampling}, we assume client samplings satisfying such that $\exists\alpha \ge 0,\ \forall i\neq j,\  \COV{\omega_i(S_t)}{\omega_j(S_t)} = - \alpha p_i p_j$. To further show the generality of this hypothesis, we provide in Appendix \ref{app:sampling_calculus}, other client samplings satisfying this condition based on a Binomial or Poisson Binomial distribution. However, these two client samplings only sample $m$ clients in expectation and thus do not have real practical use.

%\textbf{Binomial sampling}. We introduce with Binomial sampling, a client sampling where every client is sampled according to a Bernoulli with identical probability, i.e.
%\begin{equation}
%	\omega_i(S_t)
%	= \mathbb{B}(\frac{m}{n})\frac{n}{m}p_i.
%\end{equation}
%In expectation, the server always selects $m$ different clients. By design, up to $n$ different clients can be sampled and $m$ is not a bound like for MD and Uniform sampling. 



%\textbf{Clustered sampling}. [US] generalizes MD sampling by considering $m$ different distributions to sample clients from instead of the same one with MD sampling. Equation (\ref{eq:MD_aggreg_weight}) remains valid for clustered sampling with $p(\{l_k = i\}) = r_{k, i}$  where $\{r_{k, i}\}$ are the probabilities of client $i$ to be sampled in distribution $k$ and are chosen such that clustered sampling satisfies Definition \ref{def:sampling}. We note that clustered sampling does not satisfy Lemma \ref{lem:equality_update_without_Jenken} because of its covariance expression. Still, we show in Appendix \ref{app:clustered_sampling}, that the same convergence upper bound as the one for MD sampling in Theorem \ref{theo:convergence_2} holds for clustered sampling with $\delta_i(Cl) \le \delta_i(MD)$ with equality if and only if $Cl = MD$. We note that we do not provide a close form of $\delta_i(Cl)$. Like [US] who do not provide the influence of $\{r_{k, i}\}$ on FL convergence guarantees. Therefore, a reasoning behind possible induction of bias through $\delta_i(Cl)$ is not possible and is beyond the scope of this work.





%To this end, we investigate MD sampling \cite{FedProx}  the current default client sampling and Uniform sampling XXX outperforming MD sampling but that can only be used for $p_i = 1/n$. By sampling $m$ clients with replacement, with MD sampling, the server only consider up to $m$ clients. 
%%Hence, we propose IMD - Improved MD - sampling always sampling $m$ different clients based on a multinomial distribution with stopping time when $m$ different clients are considered. 
%Uniform sampling outperforms $MD$ by its sampling clients without replacement aspect. We generalize in this section Uniform sampling to any global loss function (\ref{eq:global_loss}), e.g. $p_i = n_i / M$. Finally, we consider clustered sampling XXX where $m$ clients are sampled according to $m$ different distributions. We show that Theorem \ref{theo:convergence_2} upper bound still hold despite clustered sampling covariance structure. 






%\subsection{Uniform sampling}
%
%To tackle the replacement drawback of sampling $m$ clients with MD sampling, Uniform sampling was proposed where $m$ clients are sampled without replacement. To satisfy Assumption \ref{ass:sampling} while respecting $\forall S_t,\ \sum_{i=1}^{n}\omega_i(S_t) = 1$, Uniform sampling can only be used for applications where every client is given identical importance, i.e. $p_i = 1/n$ like for a balanced federated dataset. We note that for such a federated setting, the probability for a client to be sampled is $ p (\{i \in S_t\}) = m/n$ which leads to:
%\begin{equation}
%\omega_i(S_t) 
%= \frac{\{ i \in S_t\}}{m} .
%\end{equation}
%The generalization of the aggregation process, equation (\ref{eq:aggreg_SCAFFOLD_general}), enables consideration of client sampling such that $\exists S_t,\ \sum_{i=1}^{n}\omega_i(S_t) \neq 1$. As a result, Uniform sampling can be generalized to federated loss functions where clients receive custom weights, e.g. $p_i = n_i / M$, by rescaling the stochastic aggregation weight as:
%\begin{equation}
%\omega_i(S_t) 
%= \{ i \in S_t\} \frac{n}{m}p_i.
%\end{equation}
%We note that for $p_i = 1/n$, we retrieve the Uniform sampling currently used when giving identical importance to all the clients.

%\subsection{Clustered sampling}
%
%To improve MD sampling, [US] introduces clustered sampling where $m$ clients are sampled from $m$ different distributions instead of the same one for MD sampling. As a result, MD sampling is a special clustered sampling where the $m$ distributions are identical. For clustered sampling the stochastic aggregation weight expression remains identical to the one of MD sampling, equation (\ref{eq:MD_aggreg_weight}). Instead $p(\{l_k = i\}) = r_{k, i}$  where the $\{r_{k, i}\}$ are chosen such that Assumption \ref{ass:sampling} is satisfied. 
%
%We note that clustered sampling does not satisfy Lemma \ref{lem:equality_update_without_Jenken} because of its covariance expression. Still, we show in Appendix \ref{app:clustered_sampling}, that the same convergence upper bound as the one for MD sampling in Theorem \ref{theo:convergence_2} holds for clustered sampling with $\delta_i(Cl) \le \delta_i(MD)$ with equality if and only if $Cl = MD$. We note that we do not provide a close form of $\delta_i(Cl)$. Like [US] who do not provide the influence of $\{r_{k, i}\}$ on FL convergence guarantees. Therefore, a reasoning behind possible induction of bias through $\delta_i(Cl)$ is not possible and is beyond the scope of this work.


%\subsection{Other clients sampling}
%We devise two other clients sampling in Appendix \ref{app:sampling_calculus} from a Poisson Binomial and a Binomial distribution. With these two sampling schemes, we show that clients sampling with $\alpha = 0$ exists. However, these clients samplings do not have aggregation weights summing to 1 and the amount of clients the server communicates with at every iteration is equal to $m$ only in expectation. 























==> tex/different_samplings_appednix.tex <==
\newpage

\section{Sampling schemes calculus}\label{app:sampling_calculus}

\subsection{No sampling scheme}
With no sampling scheme, all the clients are considered at every iteration. As a result, we get: $\omega_i(S_t) = p_i$ which gives $\VARR{S_t}{\omega_i(S_t)} =0$ and $\alpha = 0$ leading to:
\begin{equation}
\delta_{all}^* = 1 - \gamma^* .
\end{equation}



\subsection{MD sampling}
With MD sampling, we consider $l_1, ..., l_m$ to be the $m$ iid sampled clients from a multinomial distribution with support on $\{1, ..., m\}$ satisfying $\mathbb{P}(l=i) = p_i$ and $\sum_{i=1}^{n}p_i =1$. Hence, we get:
\begin{equation}
\omega_i(S_t) = \frac{1}{m} \sum_{k =1 }^m \{l_k = i\}
\end{equation}
Hence, we get:
%\begin{equation}
%	\VARR{S_t}{\omega_i(S_t)} =\frac{1}{m}p_i (1- p_i)
%\end{equation}
%and 
\begin{equation}
\COV{\omega_j(S_t)}{\omega_k(S_t)} = \left[ \frac{m (m-1)}{m^2} - 1 \right] p_j p_k = -\frac{1}{m} p_j p_k
\Rightarrow \alpha_{M} = - \frac{1}{m},
\end{equation}
and 
\begin{equation}
\VAR{\omega_i(S_t)} 
= \frac{1}{m^2} m p_i (1- p_i) 
= - \frac{1}{m} p_i^2 + \frac{1}{m}p_i 
\end{equation}
%which leads to 
%\begin{equation}
%\delta^* 
%= \frac{1}{m} + (1 - \gamma^*) (1 - \frac{1}{m}) 
%= 1 - \gamma^* (1 - \frac{1}{m}) 
%> \delta_{all}^*.
%\end{equation}

\subsection{ Improved MD sampling}
With Improved MD sampling, the cardinal of $|S_t|$ is stochastic and we have $|S_t| \ge m$ such that exactly $m$ different clients are sampled. Hence, we consider $l_1, ..., l_{|S_t|}$ to be the sampled clients indices from a multinomial distribution with support on $\{1, ..., m\}$ satisfying $\mathbb{P}(l=i) = p_i$ and $\sum_{i=1}^{n}p_i =1$. Hence, we get:
\begin{equation}
\omega_i(S_t) = \frac{1}{|S_t|} \sum_{k =1 }^|S_t| \{l_k = i\},
\end{equation}
where $m$ the amount of different sampled clients is hidden in $|S_t|$. The improved MD sampling is a generalization of MD sampling with $|S_t| = m$. We obtain similar results as for MD sampling by conditioning on the cardinal of $S_t$:
%\begin{equation}
%	\VARR{S_t}{\omega_i(S_t)} =\frac{1}{m}p_i (1- p_i)
%\end{equation}
%and 
\begin{equation}
\COV{\omega_j(S_t)}{\omega_k(S_t)} = \left[ \EE{|S_t|}{\frac{|S_t| (|S_t|-1)}{|S_t|^2}} - 1 \right] p_j p_k = -\E{|S_t|^{-1}} p_j p_k
\Rightarrow \alpha_{I} = - \E{|S_t|^{-1}},
\end{equation}
and 
\begin{equation}
\VAR{\omega_i(S_t)} 
= \E{\frac{1}{|S_t|^2} |S_t|} p_i (1- p_i) 
= - \E{|S_t|^{-1}} p_i^2 + \E{|S_t|^{-1}} p_i 
\end{equation}
%which leads to 
%\begin{equation}
%\delta^* 
%= \frac{1}{m} + (1 - \gamma^*) (1 - \frac{1}{m}) 
%= 1 - \gamma^* (1 - \frac{1}{m}) 
%> \delta_{all}^*.
%\end{equation}



\subsection{Uniform sampling for balanced federated dataset}
With a balanced federated dataset, i.e. $p_i = 1/n$. $m$ clients are uniformly sampled without replacement. We note that the probability for a client to be sampled is then $ p (\{i \in S_t\}) = \frac{m}{n}$. To ensure Assumption \ref{ass:sampling}, each client aggregation weight is defined as:
\begin{equation}
\omega_i(S_t) 
= \frac{\{ i \in S_t\}}{m} .
\end{equation}
We generalize the uniform sampling scheme with:
\begin{equation}
\omega_i(S_t) 
= \{ i \in S_t\} \frac{n}{m}p_i.
\end{equation}
This generalized sampling scheme satisfies Assumption \ref{ass:sampling}. We note that if the federated dataset is balanced, i.e. $p_i = 1/n$, we retrieve the uniform sampling discussed before. We also note that the sum of the stochastic aggregation weights is always equal to 1 only if the federated dataset is balanced.

In that case, we get: 
\begin{equation}
\VARR{S_t}{\omega_i(S_t)} 
=\left[\frac{n}{m}p_i\right]^2\VAR{i \in S_t}
=\frac{n}{m} (1- \frac{m}{n})p_i^2 
\Rightarrow 
a_1 = \frac{n}{m} -1 
\text{ and } 
a_2 =0,
\end{equation}
and 
\begin{equation}
\COV{\omega_j(S_t)}{\omega_k(S_t)} 
= \frac{n^2}{m^2}\frac{m (m-1)}{n(n-1)}p_j p_k - p_j p_k
\Rightarrow 
\alpha_U
 =\frac{m-1}{m} \frac{n}{n-1} - 1
 <0,
\end{equation}
which gives:
\begin{equation}
\delta_U^* 
= \frac{n}{m}(1 - \frac{m-1}{n-1})p_{max} + (1 - \gamma^*)\frac{m-1}{m}\frac{n}{n-1}.
\end{equation}



\subsection{Binomial Distribution}
Each client is sampled according to a Bernoulli distribution with identical probability, i.e.
\begin{equation}
\omega_i(S_t) 
= \frac{n}{m}\mathbb{B}(\frac{m}{n})p_i
\end{equation}
which satisfies Assumption \ref{ass:sampling}. We note that for balanced and unbalanced federated datasets, the sum of the stochastic aggregation weights is never always equal to 1. 

With MD sampling, the server communicates with at most $m$ clients, and with Uniform sampling, the server communicates with exactly $m$ clients. However, with Binomial distribution, the amount of sampled clients is stochastic and can only be bounded by $n$ with probability 1.

With Binomial distribution, we get: 
\begin{equation}
\VARR{S_t}{\omega_i(S_t)} 
=\frac{n^2}{m^2} \frac{m}{n}  (1- \frac{m}{n}) p_i^2
=\frac{n-m}{m} p_i^2 
\Rightarrow
a_1 = \frac{n-m}{m}
\text{ and }
a_2 =0
\end{equation}
and, due to the independence of each stochastic weight, we have:
\begin{equation}
\COV{\omega_j(S_t)}{\omega_k(S_t)} = \alpha = 0 
\end{equation}
which leads to 
\begin{equation}
\delta_B^* 
= \frac{n-m}{m} p_{max} + 1 - \gamma^*.
\end{equation}

\subsection{Sampling schemes comparison}

We show in the appendix that the Uniform sampling outperforms in convergence speed the uniform sampling if 

\begin{equation}
	\delta_U^* \le \delta_M^*
	\Leftrightarrow
	\gamma^* \ge
	\frac{n-m}{m-1}\left[n p_{max} -1\right]
\end{equation}
We retrieve in the balanced setting, i.e. $p_{max} = 1/n$ that uniform sampling outperforms MD sampling for any federated dataset heterogeneity in convergence speed.

Similarly for Binomial sampling, we have:
\begin{equation}
\delta_B^* \le \delta_M^*
\Leftrightarrow
\gamma^* \ge
(n-m)p_{max}
\ge \frac{n-m}{n}
\end{equation}
Hence, Binomial sampling outperforms MD sampling in rare cases. 

























==> tex/include_bias.tex <==
\section{Include Bias in the error bound}

\begin{lemma}[\cite{FedNova}] \label{lem:include_bias}
	For any model parameters $\theta$, the difference between the gradients of $\Lcal(\theta)$ and $\tilde{\Lcal}(\theta)$ can be bounded as follow:
	\begin{equation}
	\norm{\nabla \Lcal(\theta) - \tilde{\Lcal}(\theta)}^2
	\le \chi_{p ||d}^2 \left[(\beta^2 - 1) \norm{\nabla\tilde{\Lcal}(\theta)}^2  + \kappa^2 \right],
	\end{equation}
	where $\chi_{p ||d}^2$ denote the chi-square distance between $p$ and $d$, i.e. $\chi_{p ||d}^2 = \sum_{i=1}^{n} (p_i - d_i)^2/d_i$.
\end{lemma}

\begin{proof}
	According ot the definition of $\Lcal(\theta)$ and $\tilde{\Lcal}(\theta)$, we have:
	\begin{align}
		\nabla \Lcal(\theta) - \tilde{\Lcal}(\theta)
		& = \sum_{i=1}^{n} (p_i - d_i) \nabla \Lcal_i(\theta)\\
		& = \sum_{i=1}^{n} (p_i - d_i) [\nabla \Lcal_i(\theta) -  \nabla\tilde{\Lcal}(\theta)]\\
		& = \sum_{i=1}^{n} \frac{p_i - d_i}{\sqrt{d_i}} \sqrt{d_i}[\nabla \Lcal_i(\theta) -  \nabla\tilde{\Lcal}(\theta)]\\
	\end{align}
	
	Applying Cauchy-Schwartz inequality, it follows that:
	\begin{align}
		\norm{\nabla \Lcal(\theta) - \tilde{\Lcal}(\theta)}^2
		& \le \left[\sum_{i=1}^{n} \frac{(p_i - d_i)^2}{d_i}  \right] \sum_{i=1}^{n} d_i [\nabla \Lcal_i(\theta) -  \nabla\tilde{\Lcal}(\theta)]\\
		& \le \chi_{p ||d}^2 \left[(\beta^2 - 1) \norm{\nabla\tilde{\Lcal}(\theta)}^2  + \kappa^2 \right],
	\end{align}
	where the last inequality follows from Assumption \ref{ass:dissimilarity}.
\end{proof}

\begin{proof}
	We note that using Lemma \ref{lem:include_bias} and Jensen inequality, we get:
	\begin{align}
		\norm{\nabla \Lcal (\theta)}^2
		& \le 2 \norm{\nabla \Lcal ( \theta) - \nabla \tilde{\Lcal}( \theta)}^2 
		+ 2 \norm{\nabla \tilde{\Lcal}(\theta)}^2\\
		& \le 2  \left[(\beta^2 - 1) \chi_{p ||d}^2  + 1  \right] \norm{\nabla\tilde{\Lcal}(\theta)}^2  
		+ 2 \kappa^2\\
		& \le 4  \left[(\beta^2 - 1) \chi_{p ||d}^2  + 1  \right] L [\tilde{\Lcal}(\theta) - \tilde{\Lcal}(\tilde{\theta})]
		+ 2 \kappa^2
	\end{align}
	
	Hence, we have:
	\begin{align}
	\frac{1}{T}\sum_{t=0}^{T}\E{\norm{\nabla \Lcal (\theta^t)}^2}
	&  \le 4  \left[(\beta^2 - 1) \chi_{p ||d}^2  + 1  \right] L [\frac{1}{T}\sum_{t=0}^{T} [\E{\tilde{\Lcal}(\theta^t)} - \tilde{\Lcal}(\tilde{\theta})]
	+ 2 \kappa^2\\
	&  \le  4 \left[(\beta^2 - 1) \chi_{p ||d}^2  + 1  \right] L \epsilon_{opt}
	+ 2 \kappa^2\\
	\end{align}
	
\end{proof}

==> tex/method.tex <==
\section{Approach}

Current FL approaches have justified convergence through an upper bound on the global model parameters with respect to the optimal one, i.e. $\norm{x^t - x ^*}$, or with respect to the global model gradient, i.e. $\norm{\nabla F (x^t)}$. 

Overall, no convergence has been given for the variance of the learning process. The one that have takes upper bound removing the variability for clients sampling. We explain through this simple example the current flow used for the proof. We consider $\{y_j\}_{1}^J$, a subset $S$ of indices of $\{1,..., J\}$, and the quantity $\E{\norm{\sum_{j \in S}x_j}^2}$.

\begin{equation}
	\norm{\sum_{j \in S}x_j}^2
	= |S|^{2} \norm{|S|^{-1} \sum_{j \in S}x_j}^2
	\le |S| \sum_{j \in S}\norm{x_j}^2
\end{equation}


\begin{equation}
{\norm{\sum_{j \in S}x_j}^2}
= |S|^{2} \norm{|S|^{-1} \sum_{j \in S}x_j}^2
\le \left[\sum_{j \in S}\norm{x_j}\right]^2
\end{equation}

\begin{equation}
\left[\sum_{j \in S}\norm{x_j}\right]^2
= |S|^{2} \left[|S|^{-1}\sum_{j \in S}\norm{x_j}\right]^2
\le |S| \sum_{j \in S}\norm{x_j}^2
\end{equation}



\begin{equation}
	x^{t+1} 
	=  x^t + \eta \sum_{i\in S_t} (x_i^{t+1} - x^t)
\end{equation}

With MD sampling, we get:

\section{Clients sampling schemes}

\subsection{MD sampling}
\begin{lemma}\label{lem:var_MD}
	Let us consider $n$ scalars $\{y_i\}_1^n$, $n$ scalars$\{z_k\}_1^n$, and $S$ a subset of indices sampled with a multinomial distribution from $\{1, ..., n\}$ each with probability $p_i$.
	\begin{equation}
	\EE{S}{\sum_{i\in S}y_i\sum_{k\in S}z_k } = m \sum_{i=1}^{n} p_i y_i z_i + m(m-1) \sum_{i=1}^{n}\sum_{j=1}^{n}p_i p_j y_i z_j
	\end{equation}
\end{lemma}


\subsection{Poisson Binomial Distribution}


\begin{lemma}\label{lem:var_Poisson}
	Let us consider $n$ scalars $\{y_i\}_1^n$, $n$ scalars$\{z_k\}_1^n$, and $S$ a subset of indices sampled with a Poisson Binomial distribution from $\{1, ..., n\}$ each with probability $r_i$.
	\begin{equation}
	\EE{S}{\sum_{i\in S}y_i\sum_{j\in S}z_j } 
	= \sum_{i=1}^n r_i (1- r_i) y_i z_i + \sum_{i=1}^n \sum_{j = 1 }^n r_i r_j y_i z_j 
	\end{equation}
\end{lemma}


We want all the clients to have the same sampling variance. We propose therefore to consider the new aggregation scheme:
\begin{equation}
x^{t+1} 
=  x^t + \sum_{i\in S_t} \eta_i (x_i^{t+1} - x^t)
\end{equation}
Clients are still selected according to Poisson Binomial distribution. But instead of $r_i = m p_i$, All the clients are now sampled with probability $r_i = r = \frac{m}{n} $ and $\eta_i = \eta \frac{n}{m} p_i$. As a result, every client is sampled with probability 
\begin{equation}
\EE{S_t}{x^{t+1}} 
=  x^t + \EE{S_t}{\sum_{i\in S_t} \eta \frac{n}{m} p_i (x_i^{t+1} - x^t)} =  x^t + \eta \sum_{i=1}^n  p_i (x_i^{t+1} - x^t)
\end{equation}














==> tex/proof_convergence_2.tex <==







%\input{tex/sampling_properties}
%\input{tex/proofs_nips}










==> tex/proof_samplings_stats_old.tex <==
\newpage
\appendix


\section{Sampling schemes properties}

\subsection{MD sampling}
\begin{proof}
	$S$ is obtained with a multinomial distribution. We denote by $l_x$ the random variable associated to the $x^{th}$ sampled client.
	\begin{align}
	\EE{S}{\sum_{i\in S}y_i\sum_{k\in S}z_k } 
	&= \EE{S}{\sum_{i=1}^m l_i y_{l_i}\sum_{k=1}^m l_k z_{l_k} } \\
	&= \sum_{i=1}^m  \sum_{k=1}^m \EE{S}{l_i y_{l_i}l_k z_{l_k} } \\
	&= \sum_{i=1}^m  \sum_{k=1}^m \EE{S}{\sum_{j=1}^{n}\{l_i=j\} y_j \sum_{l=1}^{n} \{l_k = l\} z_l } \\
	&= \sum_{i=1}^m  \sum_{k=1}^m \sum_{j=1}^{n}\sum_{l=1}^{n}\EE{S}{\{l_i=j\} \{l_k = l\} }y_j z_l 
	\end{align}
	We have now two cases. The case where $i=k$. In that case, $\{l_i=j\}\{l_k=l\}= 0$ if $j \neq l$. Thus,we get:
	\begin{align}
	\EE{S}{\sum_{i\in S}y_i\sum_{k\in S}z_k } 
	%	&= \EE{S}{\sum_{i=1}^m l_i y_{l_i}\sum_{k=1}^m l_k z_{l_k} } \\
	%	&= \sum_{i=1}^m  \sum_{k=1}^m \EE{S}{l_i y_{l_i}l_k z_{l_k} } \\
	&= \sum_{i=1}^m  \sum_{j=1}^{n} p_j y_j z_j + \sum_{i=1}^m  \sum_{k=1, k \neq i}^m \sum_{j=1}^{n}\sum_{l=1}^{n}p_j p_l y_j z_l \\
	&= m \sum_{j=1}^{n} p_j y_j z_j + m(m-1) \sum_{j=1}^{n}\sum_{l=1}^{n}p_j p_l y_j z_l 
	%	&= \sum_{i=1}^m  \sum_{k=1}^m \EE{S}{\sum_{j=1}^{n}\{l_i=j\} y_j \sum_{l=1}^{m} \{l_k = l\} z_l } \\
	%	&= \sum_{i=1}^m  \sum_{k=1}^m \EE{S}{\sum_{j=1}^{n}\{l_i=j\} \sum_{l=1}^{m} \{l_k = l\} }y_j z_l \\
	\end{align}
\end{proof}


\subsection{Poisson Binomial Distribution}
\begin{proof}
	$S$ is obtained with a Poisson binomial distribution. 
	\begin{align}
	\EE{S}{\sum_{i\in S}y_i\sum_{k\in S}z_k }
	& = \EE{S}{\sum_{i=1}^n \mathbb{B}(r_i) y_i\sum_{k = 1}^n \mathbb{B}(r_k)z_k } \\
	& = \sum_{i=1}^n \sum_{k = 1}^n \EE{S}{\mathbb{B}(r_i) \mathbb{B}(r_k)}y_i z_k 
	\end{align}
	When, $i=j$, $\mathbb{B}(r_i) \mathbb{B}(r_j) = \mathbb{B}(r_i)$. Thus, we get:
	\begin{align}
	\EE{S}{\sum_{i\in S}y_i\sum_{j\in S}z_j }
	& = \sum_{i=1}^n \EE{S}{\mathbb{B}(r_i)}y_i z_i + \sum_{i=1}^n \sum_{j = 1, j \neq i}^n \EE{S}{\mathbb{B}(r_i) \mathbb{B}(r_j)}y_i z_j \\
	& = \sum_{i=1}^n r_i y_i z_i + \sum_{i=1}^n \sum_{j = 1, j \neq i}^n r_i r_j y_i z_j \\
	& = \sum_{i=1}^n r_i (1- r_i) y_i z_i + \sum_{i=1}^n \sum_{j = 1 }^n r_i r_j y_i z_j 
	\end{align}
\end{proof}




%\section{Convergence for any unbiased sampling scheme}
%
%Explain the framework
%
%We consider a unique $\eta_i$ for each client but we are always unbiased.
%
%
%\subsection{Lemma}
%
%\begin{lemma}
%	Suppose our local loss functions satisfy Assumptions XXX, then the local model drift from the global model can be bounded with 
%	\begin{equation}
%	\E{ \norm{y_{i, k} - x^t}^2} 
%	\le 2K^2 \eta_l^2 B^2 \E{\norm{\nabla f(x^t)}^2} + 2 K^2 \eta_l^2(\kappa^2 + \sigma^2) 
%	\end{equation}
%	
%	
%\end{lemma}
%
%\begin{proof}
%	if $K=1$, the lemma trivially holds. Thus, we consider $K\ge 2$. 
%	\begin{align}
%	\E{ \norm{y_{i, k} - x^t}^2}
%	&= \E{ \norm{y_{i, k-1} - x^t - \eta_l g_i(y_{i, k-1})}^2} \\
%	&\le (1 - \frac{1}{K-1})\E{ \norm{y_{i, k-1} - x^t}^2} + K\eta_l^2 \E{\norm{g_i(y_{i, k-1})}^2} \\
%	&\le (1 - \frac{1}{K-1})\E{ \norm{y_{i, k-1} - x^t}^2} + K\eta_l^2 [\E{\norm{\nabla f_i(y_{i, k-1})}^2} + \sigma^2]\\
%%	&\le \E{ \norm{y_{i, k-1} - x^t - \eta_l \nabla f_i(y_{i, k-1})}^2} + \eta_l \sigma^2\\
%%	&\le (1 - \frac{1}{K-1})\E{ \norm{y_{i, k-1} - x^t}^2} + \frac{\eta_l^2}{K} \E{\norm{\nabla f_i(y_{i, k-1})}^2} + \eta_l \sigma^2\\
%	&\le (1 - \frac{1}{K-1})\E{ \norm{y_{i, k-1} - x^t}^2} \nonumber \\
%	& + K \eta_l^2 \left[ 2\E{\norm{\nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)}^2}  + 2\E{\norm{\nabla f_i(x^t)}^2} + \sigma^2 \right] \\
%	&\le (1 - \frac{1}{K-1} + 2 K \eta_l^2\beta^2)\E{ \norm{y_{i, k-1} - x^t}^2} 
%	+ 2 K \eta_l^2B^2 \E{\norm{\nabla f(x^t)}^2} \nonumber\\	
%	& + 2 K \eta_l^2[\kappa^2 + \sigma^2]		
%	\end{align}
%	
%	We consider a local learning rate $\eta_l$ satisfying $\eta_l \le \frac{1}{\sqrt{2}K\beta}$ which gives $1 - \frac{1}{K-1} + 2 K \eta_l^2 \le 1$, leading to 
%	
%	\begin{align}
%	\E{ \norm{y_{i, k} - x^t}^2} 
%	&= \sum_{\tau=1}^{k} \left( 1 - \frac{1}{K-1} + \frac{2\eta_l^2\beta^2}{K}\right)^\tau \left[2K \eta_l^2 B^2 \E{\norm{\nabla f(x^t)}^2} + 2 K \eta_l^2(\kappa^2 + \sigma^2) \right]\\
%	&\le k \left[2K \eta_l^2 B^2 \E{\norm{\nabla f(x^t)}^2} + 2 K \eta_l^2(\kappa^2 + \sigma^2) \right]\\
%	&\le 2K^2 \eta_l^2 B^2 \E{\norm{\nabla f(x^t)}^2} + 2 K^2 \eta_l^2(\kappa^2 + \sigma^2) 
%	\end{align}
%\end{proof}
%
%
%\begin{lemma}
%	\begin{equation}
%	\E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \nabla f_i(y_{i, k-1})}^2}
%	\end{equation}
%\end{lemma}
%
%\begin{proof}
%	\begin{align}
%	A
%	& = \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \nabla f_i(y_{i, k-1})}^2}\\
%	&\le 2 \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \left [ \nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)\right]}^2} + 2 \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \nabla f_i(x^t)}^2}\\
%	&\le 2 \E{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)}^2} + 2 \E{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(x^t)}^2}\\
%	&\le \frac{2 \beta^2 }{K m} {\E{ \sum_{k, i\in S_t} \eta_i \norm{y_{i, k-1} - x^t}^2}} 
%	+ \frac{2}{K m} {\E{ \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(x^t)}^2}}\\
%	&\le \frac{2 \beta^2 }{K m} \sum_{k, i}p_i\underbrace{\E{  \norm{y_{i, k-1} - x^t}^2}}_{A_1} 
%	+ \frac{2}{m} \sum_{i} p_i\underbrace{\E{  \norm{\nabla f_i(x^t)}^2}}_{A_2}
%	\end{align}
%	We bound $A_1$ using Lemma XX and $A_2$ using Assumption XXX, which gives:
%	\begin{align}
%	A
%	&\le \frac{2 \beta^2 }{K m} K [2K^2 \eta_l^2 B^2 \E{\norm{\nabla f(x^t)}^2} + 2 K^2 \eta_l^2(\kappa^2 + \sigma^2)  ]
%	+ \frac{2}{m} [B^2 \E{  \norm{\nabla f(x^t)}^2} + \kappa^2]\\
%	&= \frac{2 B^2 }{m}[2K^2 \beta^2 \eta_l^2 + 1] \E{\norm{\nabla f(x^t)}^2} + \frac{2}{m}[2 \beta^2 K^2 \eta_l^2(\kappa^2 + \sigma^2) + \kappa^2]\\
%	& \le \frac{4 B^2 }{m} \E{\norm{\nabla f(x^t)}^2} + \frac{2}{m}[ 2\kappa^2 + \sigma^2]\\	
%	\end{align}
%	
%\end{proof}
%
%\subsection{Proof of Theorem XXX}
%
%
%
%
%\section{Impact of sampling variance on convergence bound}
%
%\subsection{Rewritting Lemma XX}
%
%	\begin{lemma}
%	Let us consider $y_1, ..., y_n$, $n$ scalars and assume that $S_t$, the set of sampled clients, has a distribution satisfying
%	\begin{equation}
%	\E{\sum_{i\in S_t} y_i \sum_{j\in S_t} y_j} = \sum_{i=1}^{n}\alpha_i y_i^2 + \sum_{i=1}^{n} \sum_{i=1}^{n}\beta_i \beta_j y_i,
%	\end{equation}
%	where $\alpha_i$, and $\beta_i$ are scalars. We show in that case that:
%	\begin{equation}
%	\E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \nabla f_i(y_{i, k-1})}^2} \le 
%	\end{equation}
%\end{lemma}
%
%\begin{proof}
%	\begin{align}
%	A
%	& = \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \nabla f_i(y_{i, k-1})}^2}\\
%	&\le 2 \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i\left [ \nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)\right]}^2} + 2 \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t}\eta_i \nabla f_i(x^t)}^2}\\
%	&\le 2\frac{1}{K} \sum_{k=1}^{K} \E{\norm{\frac{1}{m} \sum_{i\in S_t} \eta_i\left [ \nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)\right]}^2}
%	+ 2 \E{\norm{\frac{1}{m} \sum_{i\in S_t}\eta_i \nabla f_i(x^t)}^2}\\
%	&\le 2\frac{1}{K} \sum_{k=1}^{K} \underbrace{\E{\left(\frac{1}{m} \sum_{i\in S_t} \eta_i\norm{ \nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)}\right)^2}}_{B} 
%	+ 2 \underbrace{\E{\left(\frac{1}{m} \sum_{i\in S_t}\eta_i \norm{\nabla f_i(x^t)}\right)^2}}_C
%%	&\le 2 \E{\left(\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)}\right)^2} 
%%	+ 2 \E{\left(\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(x^t)}\right)^2}\\
%%	&\le \frac{2 \beta^2 }{K^2 m^2} {\E{ \sum_{k, i\in S_t} \eta_i \norm{y_{i, k-1} - x^t}\sum_{l, j\in S_t} \eta_j \norm{y_{j, l-1} - x^t}}} \nonumber\\
%%	&+ \frac{2}{K^2 m^2} {\E{ \sum_{k, i\in S_t} \eta_i\norm{\nabla f_i(x^t)}\sum_{l, j\in S_t} \eta_j \norm{\nabla f_j(x^t)}}}
%	\end{align}
%	
%	Let us first bound $C$. We will bound $B$ with the same process.
%	\begin{align}
%		B 
%		&= \EE{x^t, S_t}{\left(\sum_{i\in S_t} \omega_i(S_t)\norm{ \nabla f_i(x^t)}\right)^2}\\
%		&= \VARR{x^t, S_t}{\sum_{i\in S_t} \omega_i(S_t)\norm{ \nabla f_i(x^t)}} + \EE{x^t, S_t}{\sum_{i\in S_t} \omega_i(S_t)\norm{ \nabla f_i(x^t)}}^2\\
%		&= \underbrace{\VARR{x^t, S_t}{\sum_{i\in S_t} \omega_i(S_t)\norm{ \nabla f_i(x^t)}}}_D
%		+ \left[\sum_{i=1}^n p_i \EE{x^t}{\norm{ \nabla f_i(x^t)}}\right]^2
%	\end{align}
%	By using the law of total variance, we bound $D$ as
%	\begin{align}
%	D
%	&= \EE{x^t}{\VARR{S_t}{\sum_{i\in S_t} \omega_i(S_t)\norm{ \nabla f_i(x^t)}}} +  \VARR{x^t}{\EE{S_t}{\sum_{i\in S_t} \omega_i(S_t)\norm{ \nabla f_i(x^t)}}}\\
%	&= \EE{x^t}{\VARR{S_t}{\sum_{i\in S_t} \omega_i(S_t)\norm{ \nabla f_i(x^t)}}} +  \VARR{x^t}{\sum_{i=1}^np_i \norm{ \nabla f_i(x^t)}}\\
%	\end{align}
%	
%	
%%	\begin{align}
%%	A
%%	&\le 2 \E{\left(\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)}\right)^2} 
%%	+ 2 \E{\left(\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(x^t)}\right)^2}\\
%%	&\le \frac{2 \beta^2 }{K^2 m^2} {\E{ \sum_{k, i\in S_t} \eta_i \norm{y_{i, k-1} - x^t}\sum_{l, j\in S_t} \eta_j \norm{y_{j, l-1} - x^t}}} \nonumber\\
%%	&+ \frac{2}{K^2 m^2} {\E{ \sum_{k, i\in S_t} \eta_i\norm{\nabla f_i(x^t)}\sum_{l, j\in S_t} \eta_j \norm{\nabla f_j(x^t)}}}
%%	\end{align}
%	We note that $\norm{y_{j, k-1}}\norm{y_{j, l-1}} \le \max_{i, k}(\norm{y_{i, k-1}}^2)$ and $\norm{\nabla f_i(x^t)}\norm{\nabla f_j(x^t)} \le \max_{i}(\norm{\nabla f_i(x^t)})^2$. Therefore, by considering that $x_t$ and $S_t$ are independent random variables, we get:
%	\begin{align}
%	A
%	&\le \frac{2 \beta^2 }{K^2 m^2} K^2 {\EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}} \EE{x^t}{ \max_{i, k}(\norm{y_{i, k-1}}^2)}\nonumber\\
%	&+ \frac{2}{K^2 m^2} K^2 \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}\EE{x^t}{ \max_{i}(\norm{\nabla f_i(x^t)})^2}
%	\end{align}
%	All $\EE{x^t}{ \norm{y_{i, k-1}}^2}$ and $\EE{x^t}{ \norm{\nabla f_i(x^t)}^2}$ have the same upper bound. As a result, by using Lemma XXX and Assumption XXXX, we get:
%	\begin{align}
%	A
%	&\le \frac{2 \beta^2 }{m^2} \EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}  [2K^2 \eta_l^2 B^2 \E{\norm{\nabla f(x^t)}^2} + 2 K^2 \eta_l^2(\kappa^2 + \sigma^2)] \nonumber\\
%	&+ \frac{2}{m^2} \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}[B^2 \E{ \norm{\nabla f(x^t)^2}} + \kappa^2]\\
%	&= \frac{2B^2}{m^2} [2 \beta^2K^2 \eta_l^2 + 1]\EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j} \E{\norm{\nabla f(x^t)}^2} \nonumber\\
%	&+ \frac{2}{m^2} \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}[2 K^2 \beta^2 \eta_l^2(\kappa^2 + \sigma^2) + \kappa^2]\\
%	&\le \frac{4B^2}{m^2} \EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j} \E{\norm{\nabla f(x^t)}^2} + \frac{2}{m^2} \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}[2 \kappa^2 + \sigma^2],
%	\end{align}
%	where the last inequality comes from the upper bound of the learning rate.
%\end{proof}
%
%\begin{proof}
%	\begin{align}
%	A
%	& = \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \nabla f_i(y_{i, k-1})}^2}\\
%	&\le 2 \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t} \eta_i\left [ \nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)\right]}^2} + 2 \E{\norm{\frac{1}{K m} \sum_{k, i\in S_t}\eta_i \nabla f_i(x^t)}^2}\\
%	&\le 2 \E{\left(\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(y_{i, k-1}) - \nabla f_i(x^t)}\right)^2} 
%	+ 2 \E{\left(\frac{1}{K m} \sum_{k, i\in S_t} \eta_i \norm{\nabla f_i(x^t)}\right)^2}\\
%	&\le \frac{2 \beta^2 }{K^2 m^2} {\E{ \sum_{k, i\in S_t} \eta_i \norm{y_{i, k-1} - x^t}\sum_{l, j\in S_t} \eta_j \norm{y_{j, l-1} - x^t}}} \nonumber\\
%	&+ \frac{2}{K^2 m^2} {\E{ \sum_{k, i\in S_t} \eta_i\norm{\nabla f_i(x^t)}\sum_{l, j\in S_t} \eta_j \norm{\nabla f_j(x^t)}}}
%	\end{align}
%	We note that $\norm{y_{j, k-1}}\norm{y_{j, l-1}} \le \max_{i, k}(\norm{y_{i, k-1}}^2)$ and $\norm{\nabla f_i(x^t)}\norm{\nabla f_j(x^t)} \le \max_{i}(\norm{\nabla f_i(x^t)})^2$. Therefore, by considering that $x_t$ and $S_t$ are independent random variables, we get:
%	\begin{align}
%	A
%	&\le \frac{2 \beta^2 }{K^2 m^2} K^2 {\EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}} \EE{x^t}{ \max_{i, k}(\norm{y_{i, k-1}}^2)}\nonumber\\
%	&+ \frac{2}{K^2 m^2} K^2 \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}\EE{x^t}{ \max_{i}(\norm{\nabla f_i(x^t)})^2}
%	\end{align}
%	All $\EE{x^t}{ \norm{y_{i, k-1}}^2}$ and $\EE{x^t}{ \norm{\nabla f_i(x^t)}^2}$ have the same upper bound. As a result, by using Lemma XXX and Assumption XXXX, we get:
%	\begin{align}
%	A
%	&\le \frac{2 \beta^2 }{m^2} \EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}  [2K^2 \eta_l^2 B^2 \E{\norm{\nabla f(x^t)}^2} + 2 K^2 \eta_l^2(\kappa^2 + \sigma^2)] \nonumber\\
%	&+ \frac{2}{m^2} \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}[B^2 \E{ \norm{\nabla f(x^t)^2}} + \kappa^2]\\
%	&= \frac{2B^2}{m^2} [2 \beta^2K^2 \eta_l^2 + 1]\EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j} \E{\norm{\nabla f(x^t)}^2} \nonumber\\
%	&+ \frac{2}{m^2} \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}[2 K^2 \beta^2 \eta_l^2(\kappa^2 + \sigma^2) + \kappa^2]\\
%	&\le \frac{4B^2}{m^2} \EE{S_t}{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j} \E{\norm{\nabla f(x^t)}^2} + \frac{2}{m^2} \E{ \sum_{i\in S_t} \eta_i \sum_{j\in S_t} \eta_j}[2 \kappa^2 + \sigma^2],
%	\end{align}
%	where the last inequality comes from the upper bound of the learning rate.
%\end{proof}
%
%Write why the rewritting of this bound is tighter than the original.
%
%
%\subsection{Proof of Theorem XX}
















	
	







==> tex/proof_without_bounded.tex <==
\subsection{FL convergence with XX}

\subsubsection{Bounding the client drift}

\begin{lemma}\label{lem:bounded_drift_strongly_convex}
	Under Assumption \ref{ass:smoothness} and \ref{ass:unbiased}and for a local learning rate satisfying $\eta_l \le 1/\sqrt{6} L K$, a client drift can be bounded as
	\begin{equation}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2} 
	\le 2 \eta_l^2 K^2 \sigma^2
	+ 6 \eta_l^2 K^2 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 6 \eta_l^2 K^2 \E{\norm{\nabla \Lcal_i(\theta^*)}^2} ,
	\end{equation}
	and 
	\begin{equation}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	\le 2 \eta_l^2 K^3 \sigma^2 
	+ 6 \eta_l^2 K^3 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 6 \eta_l^2 K^3 \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	.
	\end{equation}
\end{lemma}

\begin{proof}
	Proof of Lemma \ref{lem:bounded_drift_strongly_convex} is very similar ot the one of Lemma \ref{lem:bounded_drift}. Equation (\ref{app:eq:B_1}) still holds:
	\begin{equation}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2} 
	\le \eta_l^2 K^2 \sigma^2 + \eta_l^2 K \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2}.
	\label{app:eq:F_1}
	\end{equation}
	
	We can bound a gradient descent as:
	\begin{align}
	\E{\norm{\nabla \Lcal_i(y_{i,k}^t)}^2}
	& \le 3 \E{\norm{\nabla \Lcal_i(y_{i,k}^t) - \nabla \Lcal_i(\theta^t) }^2} 
	+ 3 \E{\norm{\nabla \Lcal_i(\theta^t) - \nabla \Lcal_i(\theta^*) }^2} \nonumber\\
	&+ 3 \E{\norm{\nabla \Lcal_i(\theta^*) }^2}
	\end{align}
	
	Using the local loss function $L$-smoothness, Assumption \ref{ass:smoothness}, we bound the first term as:
	\begin{equation}
	\E{\norm{\nabla \Lcal_i(y_{i,k}^t) - \nabla \Lcal_i(\theta^t) }^2} 
	\le L^2 \E{\norm{y_{i,k}^t - \theta^t }^2} 
	\end{equation}
	
	and the second term as:
	\begin{equation}
	\E{\norm{\nabla \Lcal_i(y_{k}^t) - \nabla \Lcal_i(\theta^*) }^2}
	\le L^2 \E{\norm{\theta^t - \theta^*}} 
	\end{equation}
	
	which gives:
	\begin{align}
	\E{\norm{\nabla \Lcal_i(y_{i,k}^t)}^2}
	& \le 3 L^2 \E{\norm{y_{i,k}^t - \theta^t }^2} 
	+ 3 L^2 \E{\norm{\theta^t - \theta^*}^2} 
	+ 3 \E{\norm{\nabla \Lcal_i(\theta^*) }^2}
	\label{app:eq:F_2}
	\end{align}
	
	Substituting equation (\ref{app:eq:F_2}) in equation (\ref{app:eq:F_1}), we get:
	\begin{align}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2} 
%	\E{\norm{y_{i,k}^t - \theta^t}^2}
	& \le \eta_l^2 K^2 \sigma^2 
	+ 3 \eta_l^2 K L^2 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2} \nonumber \\
	&+ 3 \eta_l^2 K^2 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 3 \eta_l^2 K^2 \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	\label{app:eq:F_3}
	\end{align}
	
	As for Lemma \ref{lem:bounded_drift}, equation (\ref{app:eq:B_5}) holds and we get:
	\begin{align}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	& \stackrel{(\ref{app:eq:B_5})}{\le} \eta_l^2 K^3 \sigma^2 + \eta_l^2 K^2 \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2}\\
	& \stackrel{(\ref{app:eq:F_2})}{\le} \eta_l^2 K^3 \sigma^2 
	 + 3 \eta_l^2 K^2 L^2 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2} \nonumber \\
	&+ 3 \eta_l^2 K^3 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 3 \eta_l^2 K^3 \E{\norm{\nabla \Lcal_i(\theta^*)}^2} ,
	\end{align}	
	
	We consider $\eta_l \le 1/\sqrt{6}KL$ which implies that $1 - 3 \eta_l^2 K^2 L^2 \ge 1/2$ giving :
	\begin{equation}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	\le 2 \eta_l^2 K^3 \sigma^2 
	+ 6 \eta_l^2 K^3 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 6 \eta_l^2 K^3 \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	\label{app:eq:F_4}
	\end{equation}
	
	Considering $\eta_l \le 1/\sqrt{6}KL$ and substituting equation (\ref{app:eq:F_4}) in equation (\ref{app:eq:F_3}) completes the proof.
\end{proof}


\subsection{Proof of Theorem \ref{theo:convergence_paper}}\label{app:proof:convergence_2}

%\begin{theorem}[FL convergence without Assumption \ref{ass:dissimilarity} or \ref{ass:bounded_gradient}]\label{theo:convergence_2}
%	Under Assumptions \ref{ass:smoothness} to \ref{ass:unbiased}, with $\mu$-strongly convex local loss functions, with small enough local step size $\eta_l = \sqrt{m/KT}$, and clients sampling satisfying Definition \ref{def:sampling} with $\COV{\omega_j(S_t)}{\omega_k(S_t)} = \alpha p_j p_k \le 0$, we get the following convergence bound:
%	\begin{align}
%	\frac{1}{T+1}\sum_{t=0}^{T}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
%	& \le \Ocal(\frac{1}{\eta_g\sqrt{m K T}}) 
%	+ \Ocal(\frac{mK}{T}) 
%	+ \Ocal( \sqrt{\frac{mK }{ T }} \eta_g\VAR{\sum_{i=1}^{n}\omega_i(S_t)}) \nonumber\\
%	&+ \Ocal(\sqrt{\frac{mK }{ T }} \eta_g  \sum_{i=1}^{n}\delta_i \EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}),
%	\label{eq:convergence_2}
%	\end{align}	
%	where $\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}$ is the optimum model $\theta^*$ performance evaluated on the local loss function $\Lcal_i$ with batch $\xi_i$.
%\end{theorem}


\begin{proof}
	By substituting $\EE{t}{\theta_i^{t+1} - \theta^t} = \sum_{k=0}^{K-1} \EE{t}{\nabla \Lcal(y_{i, k}^t)}$ in equation (\ref{eq:one_server_iteration_bound}), we get:
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	\underbrace{- 2 \tilde{\eta} \inner{\sum_{k, i}p_i \nabla \Lcal_i(y_{i,k}^t)}{\theta^t - \theta^*}}_{T_1} + \underbrace{\eta_g^2 \sum_{i=1}^{n}\delta_i\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 }}_{T_2},  \label{app:eq:G_1}
	\end{align}
%	with 
%	\begin{equation}
%	\delta_i 
%	= \VARR{S_t}{\omega_i(S_t)} - \alpha p_i^2 + (1 - \gamma^t)(1+ \alpha) p_i .
%	\end{equation}
	
	
	
	\subsubsection*{Bounding $T_1$}
	Using Lemma \ref{lem:perturbed_strong_convexity} with $\mu$ strongly convex functions, we can bound $T_1$ as :
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} \sum_{k, i}p_i \left[ \Lcal_i(\theta^t) - \Lcal_i(\theta^*) - L \EE{t}{\norm{y_{i, k}^t - \theta^t}^2}
			+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right]\\
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
			+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] + 2 L \tilde{\eta} \sum_{i}p_i\sum_{k}\EE{t}{\norm{y_{i,k}^t - \theta^t}^2},
	\end{align}
	where $\sum_{k} \EE{t}{\norm{y_{i,k}^t - \theta^t}^2}$ can be bounded using Lemma \ref{lem:bounded_drift_strongly_convex}:
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
		+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] \nonumber\\
	&+ 4 \eta_l^2 \tilde{\eta} K^3 L \sigma^2 
	+ 12 \eta_l^2 \tilde{\eta} K^3 L^3 \norm{\theta^t - \theta^*}^2
	+ 12 \eta_l^2 \tilde{\eta} K^3 L \sum_{i=1}^{n}p_i\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2} \nonumber\\
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right]
	 - \left[\tilde{\eta} K\frac{\mu}{2} - 12 \eta_l^2 \tilde{\eta} K^3 L^3 \right]\norm{\theta^t - \theta^*}^2
	 + \gamma,
	\label{app:eq:G_2}
	\end{align}
	where $\gamma = 4 \eta_l^2 \tilde{\eta} K^3 L \sigma^2 
	+ 12 \eta_l^2 \tilde{\eta} K^3 L \sum_{i=1}^{n}p_i\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}$.
	
	
	
	
	
	
	\subsubsection*{Bounding $T_2$}	
	$\delta = \sum_{i=1}^{n} \delta_i$ and we define $\epsilon = \sum_{i=1}^{n}\delta_i \EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}$. Using Lemma \ref{lem:bounded_drift} to bound $\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 } $,we get:
	\begin{align}
	T_2 
	&\le 2 \tilde{\eta}^2 K^2 \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2 L^2 \norm{\theta^t - \theta^*}^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon,
	\label{app:eq:G_3}
	\end{align}	
	
	
	\subsubsection*{Bounding equation (\ref{app:eq:G_1})}
	Substituting equation (\ref{app:eq:G_3}) and (\ref{app:eq:G_2}) in equation (\ref{app:eq:G_1}), we get:	
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right] 
	- \left[\tilde{\eta} K\frac{\mu}{2} - 12 \eta_l^2 \tilde{\eta} K^3 L^3 \right]\norm{\theta^t - \theta^*}^2
	\nonumber\\
	&+ \gamma 
	+ 2 \tilde{\eta}^2 K^2 \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2 L^2 \norm{\theta^t - \theta^*}^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon\\
	&= \left[ 1 - \left[\tilde{\eta} K\frac{\mu}{2} - 12 \eta_l^2 \tilde{\eta} K^3 L^3 \right]+ 6 \tilde{\eta}^2 K^2 L^2 \delta\right] \norm{\theta^t - \theta^*}^2 
	\nonumber\\
	&- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right] 
	+ \gamma 
	+ 2 \tilde{\eta}^2 K^2 \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon
	\end{align}
	
	We consider a small enough local learning rate such that $ 1 - \tilde{\eta} K\frac{\mu}{2} + 12 \eta_l^2 \tilde{\eta} K^3 L^3 + 6 \tilde{\eta}^2 K^2 L^2 \le 1 $ which is equivalent to $ 2 \eta_l^2 KL + \eta_g \eta_l \delta - \frac{\mu}{12 K L^2} \le 0$. Hence, we get:
	\begin{equation}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	\le \norm{\theta^t - \theta^*}^2 - \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right] 
	+ \gamma 
	+ 2 \tilde{\eta}^2 K^2 \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon
	\end{equation}
	
	Finally, by rearranging the terms, and taking the expectation over all the global model history, we get:
	\begin{align}
	\E{\Lcal(\theta^t)} - \Lcal(\theta^*)
	& \le \frac{1}{\tilde{\eta} K }\left[\E{\norm{\theta^t - \theta^*}^2} 
	- \E{\norm{\theta^{t+1} - \theta^*}^2} \right]
	+ 2 \tilde{\eta} K \sigma^2 \delta
	+ 6 \tilde{\eta} K  \epsilon \nonumber \\
	& + 4 \eta_l^2 K^2 L \sigma^2 
	+ 12 \eta_l^2 K^2 L \sum_{i=1}^{n}p_i\E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	\label{app:eq:G_4}
	\end{align}
	
%	We note that 
%	\begin{align}
%	\VAR{\sum_{i=1}^{n}\omega_i(S_t)}
%	&=
%	\sum_{i=1}^{n}\VAR{\omega_i(S_t)} 
%	+ \sum_{i, j\neq i}\COV{\omega_i(S_t)}{\omega_j(S_t)}\\
%	&= \sum_{i=1}^{n}\VAR{\omega_i(S_t)} 
%	+ \alpha \sum_{i=1}^{n} p_i (1-p_i)
%	\end{align}
%	which gives:
%	\begin{equation}
%	\delta
%	= \sum_{i=1}^{n} \delta_i = \VAR{\sum_{i=1}^{n}\omega_i(S_t)} +1
%	\label{app:eq:G_5}
%	\end{equation}
	
	Summing over the global model history, we get: 
	\begin{align}
	\frac{1}{T+1}\sum_{t=0}^{T}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
	& \le \frac{1}{\tilde{\eta} K T}\E{\norm{\theta^0 - \theta^*}^2} \nonumber\\
	&+ \eta_l^2 K^2 [4L \sigma^2 
	+ 12  L \sum_{i=1}^{n}p_i\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}] 
	\nonumber \\
	&+ 2 \tilde{\eta} K \sigma^2 \delta
	+ 6 \tilde{\eta} K  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2}\\
	& = \Ocal( \frac{1}{\tilde{\eta} K T}) 
	+ \Ocal ( \eta_l^2 K^2)
	+ \Ocal(\eta_g \eta_l K \delta) \nonumber\\
	&+ \Ocal(\eta_g \eta_l K  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2})
	\end{align}	
	
%	With $\eta_l = \sqrt{m / KT}$, we get:
%	\begin{align}
%	\frac{1}{T+1}\sum_{t=0}^{T}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
%	& \le \frac{1}{\eta_g\sqrt{m K T}}\E{\norm{\theta^0 - \theta^*}^2} 
%	+ 4 \frac{mK}{T} L \sigma^2 
%	\nonumber\\
%	&+ 12 \frac{mK}{T} L \sum_{i=1}^{n}p_i\E{\norm{\nabla \Lcal_i(\theta^*)}^2} \nonumber \\
%	&+ 2 \sqrt{\frac{mK }{ T }} \eta_g \sigma^2 (\VAR{\sum_{i=1}^{n}\omega_i(S_t)} + 1)\nonumber \\
%	&+ 6 \sqrt{\frac{mK }{ T }}\eta_g  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
%	\end{align}	
	
	With $\eta_l = \sqrt{m / KT}$, we get:
	\begin{align}
	\frac{1}{T+1}\sum_{t=0}^{T+1}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
	& \le \Ocal(\frac{1}{\eta_g\sqrt{m K T}}) 
	+ \Ocal(\frac{mK}{T}) 
	+ \Ocal( \sqrt{\frac{mK }{ T }} \eta_g\VAR{\sum_{i=1}^{n}\omega_i(S_t)}) \nonumber\\
	&+ \Ocal(\sqrt{\frac{mK }{ T }} \eta_g  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2})
	\end{align}	
	
	
\end{proof}

\newpage





==> tex/proofs_nips.tex <==


\subsection{Property of convex functions}

\begin{lemma}[Perturbed strong convexity]\label{lem:perturbed_strong_convexity}
	The following holds for any $L$-smooth and $\mu$-strongly convex function $h$, and any $x$, $y$, $z$ in the domain of $h$:
	\begin{equation}
		\inner{\nabla h(x)}{z - y}
		\ge h(z) - h(y) + \frac{\mu}{4} \norm{y -z}^2 - L \norm{z - x}^2
	\end{equation}
\end{lemma}

\begin{proof}
	We use the $L$-smoothness of $h$ to get
	\begin{equation}
		\inner{\nabla h(x)}{z - x}
		\ge h(z) - h(x) - \frac{L}{2}\norm{z - x}^2,
	\end{equation}
	and the $\mu$ strong convexity to get:
	\begin{equation}
	\inner{\nabla h(x)}{x - y}
	\ge h(x) - h(y) + \frac{\mu}{2}\norm{y - x}^2.
	\end{equation}
	Applying the relaxed triangular inequality, we get:
	\begin{equation}
		\frac{\mu}{2} \norm{y-x}^2
		\ge \frac{\mu}{4} \norm{y - z}^2 - \frac{\mu}{2}\norm{x - z}
	\end{equation}
	Combining all the inequalities together, we have:
	\begin{equation}
	\inner{\nabla h(x)}{z - y}
	\ge h(z) - h(y) + \frac{\mu}{4} \norm{y -z}^2 - \frac{L + \mu}{2} \norm{z - x}^2,
	\end{equation}
	with $L\ge \mu$ which completes the proof.
\end{proof}



\subsection{FL convergence with strongly convex local loss functions}\label{app:sec:convergence_strongly_convex}

\subsubsection{Bounding a client drift}

\begin{lemma}\label{lem:bounded_drift_strongly_convex}
	Under Assumption \ref{ass:smoothness} and \ref{ass:unbiased} and for a local learning rate satisfying $\eta_l \le 1/\sqrt{6} L K$, we have

	\begin{equation}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	\le 2 \eta_l^2 K^2 \sigma^2 
	+ 6 \eta_l^2 K^3 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 6 \eta_l^2 K^3 \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	.
	\end{equation}
\end{lemma}

\begin{proof}
%	Using the same reasoning as the one to obtain on equation (\ref{app:eq:L_i}) (Corollary \ref{cor:equality_decomposition}), we get:
%	\begin{align}
%	\E{\norm{y_{i, k}^t - \theta^t}^2} 
%	& \le \eta_l^2 \E{\norm{\xi_i^t}^2} + \eta_l^2 \E{\norm{h_i^t}^2}
%	\\
%	& \le \eta_l^2 K \sigma^2 + \eta_l^2 K \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2}
%	.
%	\label{app:eq:F_1}
%	\end{align}
%	where the second inequality comes from using Assumption \ref{ass:unbiased} and Jensen inequality.
	

	We first propose the following intermediary result which bounds the gradient of model $x$ with respect to the one of the optimization problem (\ref{eq:global_loss}) optimum and the parameters of the current global model $\theta^t$:
	\begin{align}
	\E{\norm{\nabla \Lcal_i(x)}^2}
	& \le 3 \E{\norm{\nabla \Lcal_i(x) - \nabla \Lcal_i(\theta^t) }^2} 
	+ 3 \E{\norm{\nabla \Lcal_i(\theta^t) - \nabla \Lcal_i(\theta^*) }^2} \nonumber\\
	&+ 3 \E{\norm{\nabla \Lcal_i(\theta^*) }^2} \\
	& \le 3 L^2 \E{\norm{x - \theta^t }^2} 
	+ 3 L^2 \E{\norm{\theta^t - \theta^*}^2}  
	+ 3 \E{\norm{\nabla \Lcal_i(\theta^*) }^2}
	\label{app:eq:F_2}
	\end{align}
	where the last inequality comes from using the local loss function $L$-smoothness, Assumption \ref{ass:smoothness}.
	


	By construction, we have $y_{i,k}^t - \theta^t = - \sum_{l=0}^{k-1} \eta_l g_i(y_{i,l}^t)$. Following the reasoning used to derive equation (\ref{app:eq:L_i}) while using Jensen inequality and Assumption \ref{ass:unbiased}, we get:
	\begin{align}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
%	& \le \sum_{k =0}^{K-1} k \sum_{l=0}^{k -1} \eta_l^2\E{\norm{g_i(y_{i,l}^t)}^2}\\
%	& \le \eta_l^2 K^2 \sum_{k =0}^{K-1} \E{\norm{g_i(y_{i, k}^t)}^2}\\
%	& = \eta_l^2 K^2 \sum_{k=0}^{K-1} \left[ \E{\norm{g_i(y_{i,l}^t) - \nabla \Lcal_i(y_{i,l}^t)}^2}+ \E{\norm{\nabla \Lcal_i(y_{i,l}^t)}^2}\right]\\
	& \le \sum_{k=0}^{K-1} \eta_l^2 \left[  k \sigma^2 
	+ k \sum_{l=0}^{k} \E{\norm{\nabla \Lcal_i(y_{i, l}^t)}^2} \right]
	\\
	& 
%	\stackrel{A\ref{ass:unbiased}}{\le} 
	\le
	\eta_l^2 K^2 \sigma^2 + \eta_l^2 K^2 \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2}
	\end{align}	
	
	Substituting our intermediary results of equation (\ref{app:eq:F_2}) gives:	
	\begin{align}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	&\le
	\eta_l^2 K^2 \sigma^2 
	+ 3 \eta_l^2 K^2 L^2 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2} 
	\nonumber \\
	&+ 3 \eta_l^2 K^3 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 3 \eta_l^2 K^3 \E{\norm{\nabla \Lcal_i(\theta^*)}^2} ,
	\end{align}	


	
	We consider $\eta_l \le 1/\sqrt{6}KL$ which implies that $1 - 3 \eta_l^2 K^2 L^2 \ge 1/2$ giving :
	\begin{equation}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	\le 2 \eta_l^2 K^2 \sigma^2 
	+ 6 \eta_l^2 K^3 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 6 \eta_l^2 K^3 \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	,
	\label{app:eq:F_4}
	\end{equation}
	which completes the proof.
%	Considering $\eta_l \le 1/\sqrt{6}KL$ and substituting equation (\ref{app:eq:F_4}) in equation (\ref{app:eq:F_3}) completes the proof.
\end{proof}





\begin{lemma}\label{lem:bounded_hit_strongly_convex}
	Under Assumption \ref{ass:smoothness} and \ref{ass:unbiased} and for a local learning rate satisfying $\eta_l \le 1/\sqrt{6} L K$, a client drift can be bounded as
	\begin{equation}
	\E{\norm{h_i^t}^2} 
	\le K \sigma^2
	+ 6 K^2 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 6 K^2 \E{\norm{\nabla \Lcal_i(\theta^*)}^2} .
	\end{equation}

\end{lemma}

\begin{proof}
	Combining $\E{\norm{h_i^t}^2} \le  K \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2}$ with equation (\ref{app:eq:F_2}) gives:
	\begin{equation}
	\E{\norm{h_i^t}^2}  
	\le 3 K L^2 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2} 
	+ 3 K^2 L^2 \E{\norm{\theta^t - \theta^*}^2}
	+ 3 K^2 \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	\label{app:eq:F_3}
	\end{equation}
	
	Substituting Lemma \ref{lem:bounded_drift_strongly_convex} in equation (\ref{app:eq:F_3}) completes the proof.
	
\end{proof}





\subsubsection{Proof of Theorem \ref{theo:convergence_paper}}\label{app:proof:convergence_2}

%\begin{theorem}[FL convergence without Assumption \ref{ass:dissimilarity} or \ref{ass:bounded_gradient}]\label{theo:convergence_2}
%	Under Assumptions \ref{ass:smoothness} to \ref{ass:unbiased}, with $\mu$-strongly convex local loss functions, with small enough local step size $\eta_l = \sqrt{m/KT}$, and clients sampling satisfying Definition \ref{def:sampling} with $\COV{\omega_j(S_t)}{\omega_k(S_t)} = \alpha p_j p_k \le 0$, we get the following convergence bound:
%	\begin{align}
%	\frac{1}{T+1}\sum_{t=0}^{T}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
%	& \le \Ocal(\frac{1}{\eta_g\sqrt{m K T}}) 
%	+ \Ocal(\frac{mK}{T}) 
%	+ \Ocal( \sqrt{\frac{mK }{ T }} \eta_g\VAR{\sum_{i=1}^{n}\omega_i(S_t)}) \nonumber\\
%	&+ \Ocal(\sqrt{\frac{mK }{ T }} \eta_g  \sum_{i=1}^{n}\delta_i \EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}),
%	\label{eq:convergence_2}
%	\end{align}	
%	where $\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}$ is the optimum model $\theta^*$ performance evaluated on the local loss function $\Lcal_i$ with batch $\xi_i$.
%\end{theorem}


\begin{proof}
	
%	By substituting $\EE{t}{\theta_i^{t+1} - \theta^t} = \sum_{k=0}^{K-1} \EE{t}{\nabla \Lcal_i(y_{i, k}^t)}$ in equation (\ref{eq:one_server_iteration_bound})[TO CONFIRM], we get:
%	\begin{align}
%	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
%	&\le \norm{\theta^t - \theta^*}^2 
%	\underbrace{- 2 \tilde{\eta} \inner{\sum_{k, i}p_i \nabla \Lcal_i(y_{i,k}^t)}{\theta^t - \theta^*}}_{T_1} + \underbrace{\eta_g^2 \sum_{i=1}^{n}\delta_i\EE{t}{\norm{h_i^t}^2 }}_{T_2},  \label{app:eq:G_1}
%	\end{align}
	\begin{align}
	\E{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \E{\norm{\theta^t - \theta^*}^2 }
	\underbrace{- 2 \tilde{\eta} \E{\inner{\sum_{k, i}p_i \nabla \Lcal_i(y_{i,k}^t)}{\theta^t - \theta^*}}}_{T_1}
	\nonumber\\
	& + \underbrace{\tilde{\eta}^2 \sum_{i=1}^{n}\delta_i\EE{t}{\norm{h_i^t}^2 }}_{T_2}
	+ \underbrace{\tilde{\eta}^2 \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right]  \E{\norm{\xi_i^t}^2 }  }_{T_3},   \label{app:eq:G_1}
	\end{align}
	
	
	

	

	
	
	
	\subsubsection*{Bounding $T_1$}
	Using Lemma \ref{lem:perturbed_strong_convexity} with $\mu$ strongly convex functions, we can bound $T_1$ as :
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} \sum_{k, i}p_i \left[ \Lcal_i(\theta^t) - \Lcal_i(\theta^*) - L \EE{t}{\norm{y_{i, k}^t - \theta^t}^2}
			+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right]\\
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
			+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] + 2 L \tilde{\eta} \sum_{i}p_i\sum_{k}\EE{t}{\norm{y_{i,k}^t - \theta^t}^2},
	\end{align}
	where $\sum_{k} \EE{t}{\norm{y_{i,k}^t - \theta^t}^2}$ can be bounded using Lemma \ref{lem:bounded_drift_strongly_convex}:
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
		+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] \nonumber\\
	&+ 4 \eta_l^2 \tilde{\eta} K^2 L \sigma^2 
	+ 12 \eta_l^2 \tilde{\eta} K^3 L^3 \norm{\theta^t - \theta^*}^2
	+ 12 \eta_l^2 \tilde{\eta} K^3 L \sum_{i=1}^{n}p_i\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2} \nonumber\\
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right]
	 - \left[\tilde{\eta} K\frac{\mu}{2} - 12 \eta_l^2 \tilde{\eta} K^3 L^3 \right]\norm{\theta^t - \theta^*}^2
	 + \gamma,
	\label{app:eq:G_2}
	\end{align}
	where $\gamma = 4 \eta_l^2 \tilde{\eta} K^2 L \sigma^2 
	+ 12 \eta_l^2 \tilde{\eta} K^3 L \sum_{i=1}^{n}p_i\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}$.
	
	
	
	
	
	
	\subsubsection*{Bounding $T_2$}	
	$\delta = \sum_{i=1}^{n} \delta_i$ and we define $\epsilon = \sum_{i=1}^{n}\delta_i \EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}$. Using Lemma \ref{lem:bounded_hit_strongly_convex} to bound $\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 } $, we get:
	\begin{align}
	T_2 
	&\le \tilde{\eta}^2 K \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2 L^2 \norm{\theta^t - \theta^*}^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon,
	\label{app:eq:G_3}
	\end{align}	
	
	
	\subsubsection*{Bounding $T_3$}	
	Using Assumption \ref{ass:unbiased} with $\nu = \sum_{i=1}^{n} \left[ \VAR{\omega_i(S_t)} + p_i^2 \right]$, we get:
	\begin{equation}
	T_3 
	\le \tilde{\eta}^2 \nu K \sigma^2
	\end{equation} 
	
	
	
	\subsubsection*{Bounding equation (\ref{app:eq:G_1})}
	Substituting equation (\ref{app:eq:G_3}) and (\ref{app:eq:G_2}) in equation (\ref{app:eq:G_1}), we get:	
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right] 
	- \left[\tilde{\eta} K\frac{\mu}{2} - 12 \eta_l^2 \tilde{\eta} K^3 L^3 \right]\norm{\theta^t - \theta^*}^2
	\nonumber\\
	&+ \gamma 
	+ 2 \tilde{\eta}^2 K \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2 L^2 \norm{\theta^t - \theta^*}^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon
	+ \tilde{\eta}^2 \nu K \sigma^2
	\\
	&= \left[ 1 - \tilde{\eta} K \left(\frac{\mu}{2} - 12 \eta_l^2 K^2 L^3 - 6 \tilde{\eta} K L^2 \delta \right) \right] \norm{\theta^t - \theta^*}^2 
	\nonumber\\
	&- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right] 
	+ \gamma 
	+ 2 \tilde{\eta}^2 K \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon 
	+ \tilde{\eta}^2 \nu K \sigma^2
	\\
	& \le \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right] 
	+ \gamma 
	+ 2 \tilde{\eta}^2 K \sigma^2 \delta
	+ 6 \tilde{\eta}^2 K^2  \epsilon
	+ \tilde{\eta}^2 \nu K \sigma^2,
	\end{align}
	where the last inequality comes from considering a small enough local learning rate such that $ 1 - \tilde{\eta} K \left(\frac{\mu}{2} - 12 \eta_l^2 K^2 L^3 - 6 \tilde{\eta} K L^2 \delta \right) \le 1 $ which is equivalent to $ \mu - 24 \eta_l^2 K^2 L^3 - 12 \tilde{\eta} K L^2 \delta  \ge 0$. 
	
	Finally, by rearranging the terms, we get:
	\begin{align}
	\E{\Lcal(\theta^t)} - \Lcal(\theta^*)
	& \le \frac{1}{2 \tilde{\eta} K }\left[\E{\norm{\theta^t - \theta^*}^2} 
	- \E{\norm{\theta^{t+1} - \theta^*}^2} \right]
	+ \tilde{\eta} \sigma^2 \delta
	+ 3 \tilde{\eta} K  \epsilon \nonumber \\
	& + 2 \eta_l^2 K L \sigma^2 
	+ 6 \eta_l^2 K^2 L \sum_{i=1}^{n}p_i\E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	+ \frac{1}{2}\tilde{\eta} \nu \sigma^2
	\label{app:eq:G_4}
	\end{align}
	
%	We note that 
%	\begin{align}
%	\VAR{\sum_{i=1}^{n}\omega_i(S_t)}
%	&=
%	\sum_{i=1}^{n}\VAR{\omega_i(S_t)} 
%	+ \sum_{i, j\neq i}\COV{\omega_i(S_t)}{\omega_j(S_t)}\\
%	&= \sum_{i=1}^{n}\VAR{\omega_i(S_t)} 
%	+ \alpha \sum_{i=1}^{n} p_i (1-p_i)
%	\end{align}
%	which gives:
%	\begin{equation}
%	\delta
%	= \sum_{i=1}^{n} \delta_i = \VAR{\sum_{i=1}^{n}\omega_i(S_t)} +1
%	\label{app:eq:G_5}
%	\end{equation}
	
	Summing over the global model history, we get: 
	\begin{align}
	\frac{1}{T+1}\sum_{t=0}^{T}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
	& \le \frac{1}{2 \tilde{\eta} K (T+1)}\E{\norm{\theta^0 - \theta^*}^2} \nonumber\\
	&+ 6 \eta_l^2 K^2   L \sum_{i=1}^{n}p_i\EE{\xi_i}{\norm{\nabla \Lcal_i(\theta^*)}^2}] 
	\nonumber \\
	&+ \tilde{\eta} \sigma^2 \delta
	+ 2 \eta_l^2 K  L \sigma^2
	+ 3 \tilde{\eta} K  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
	\nonumber\\
	&+ \frac{1}{2}\tilde{\eta} \nu \sigma^2\\
	& = \Ocal( \frac{1}{\tilde{\eta} K T}) 
	+ \Ocal ( \eta_l^2 K^2)
	+ \Ocal(\eta_g \eta_l \left[ \delta + \nu /2 \right] \sigma^2 )
	+ \Ocal(\eta_l^2 K L \sigma^2) \nonumber\\
	&+ \Ocal(\eta_g \eta_l K  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2})
	\end{align}	
	
%	With $\eta_l = \sqrt{m / KT}$, we get:
%	\begin{align}
%	\frac{1}{T+1}\sum_{t=0}^{T}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
%	& \le \frac{1}{\eta_g\sqrt{m K T}}\E{\norm{\theta^0 - \theta^*}^2} 
%	+ 4 \frac{mK}{T} L \sigma^2 
%	\nonumber\\
%	&+ 12 \frac{mK}{T} L \sum_{i=1}^{n}p_i\E{\norm{\nabla \Lcal_i(\theta^*)}^2} \nonumber \\
%	&+ 2 \sqrt{\frac{mK }{ T }} \eta_g \sigma^2 (\VAR{\sum_{i=1}^{n}\omega_i(S_t)} + 1)\nonumber \\
%	&+ 6 \sqrt{\frac{mK }{ T }}\eta_g  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2}
%	\end{align}	
	
% 	With $\eta_l = \sqrt{m / KT}$, we get:
% 	\begin{align}
% 	\frac{1}{T+1}\sum_{t=0}^{T+1}\left[ \E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]
% 	& \le \Ocal(\frac{1}{\eta_g\sqrt{m K T}}) 
% 	+ \Ocal(\frac{mK}{T}) 
% 	+ \Ocal( \sqrt{\frac{mK }{ T }} \eta_g\VAR{\sum_{i=1}^{n}\omega_i(S_t)}) \nonumber\\
% 	&+ \Ocal(\sqrt{\frac{mK }{ T }} \eta_g  \sum_{i=1}^{n}\delta_i \E{\norm{\nabla \Lcal_i(\theta^*)}^2})
% 	\end{align}	
	
	
\end{proof}



\subsection{FL convergence with Assumption \ref{ass:dissimilarity}}\label{app:sec:convergence_ass_3}

\subsubsection{Bounding the client drift}


\begin{lemma}\label{lem:bounded_drift}
	Under Assumption \ref{ass:smoothness} and \ref{ass:unbiased}, and for a local learning rate satisfying $\eta_l \le \frac{1}{2 L K}$, a client drift can be bounded as
	\begin{equation}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2} 
	\le 2 \eta_l^2 K^2[\sigma^2 + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}], 
	\end{equation}
	and 
	\begin{equation}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	\le 2 \eta_l^2 K^3[\sigma^2 + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}].
	\end{equation}
\end{lemma}

\begin{proof}	
	By construction, we have $\theta_i^{t+1} - \theta^t = - \sum_{k=0}^{K-1} \eta_l g_i(y_{i,k}^t)$. Using Jensen's inequality, we get:
	\begin{align}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2} 
%	& \le K \sum_{k=0}^{K - 1}\E{\norm{y_{i,k}^t - \theta^t}^2}\\
%	& \le k \sum_{l=0}^{k-1} \eta_l^2\E{\norm{g_i(y_{i,l}^t)}^2}\\
	& \le K \eta_l^2 \sum_{k=0}^{K-1} \E{\norm{g_i(y_{i,k}^t)}^2}\\
	& = K \eta_l^2 \sum_{k = 0}^{K-1} \left[ \E{\norm{g_i(y_{i, k}^t) - \nabla \Lcal_i(y_{i, k}^t)}^2} + \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2}\right]\\
	& \le \eta_l^2 K^2 \sigma^2 + \eta_l^2 K \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2},
	\label{app:eq:B_1}
	\end{align}
	where the equality comes from the unbiasedness of the SGD estimator, Assumption \ref{ass:unbiased}, and the last inequality comes from the bounded variance of the SGD estimator, Assumption \ref{ass:unbiased}.
	
	In addition, we can bound a gradient descent as:
	\begin{align}
	\E{\norm{\nabla \Lcal_i(y_{i,k}^t)}^2}
	& \le 2 \E{\norm{\nabla \Lcal_i(y_{i,k}^t) - \nabla \Lcal_i(\theta^t)}^2} + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}\\
	& \le 2 L^2 \E{\norm{y_{i,k}^t - \theta^t}^2} + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2},
	\label{app:eq:B_2}
	\end{align}
	where the last inequality comes from the $L$-smoothness of the local loss functions, Assumption \ref{ass:smoothness}.
	
	Substituting equation (\ref{app:eq:B_2}) in equation (\ref{app:eq:B_1}), we get:
	\begin{align}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2} 
	& \le \eta_l^2 K^2 \sigma^2 
	+ 2 \eta_l^2 K L^2 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2} 
	+ 2 \eta_l^2 K^2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2} ,
	\label{app:eq:B_3}
	\end{align}

	By construction, we have $y_{i,k}^t - \theta^t = - \sum_{l=0}^{k-1} \eta_l g_i(y_{i,l}^t)$. Using Jensen's inequality, we get:
	\begin{align}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	& \le \sum_{k =0}^{K-1} k \sum_{l=0}^{k -1} \eta_l^2\E{\norm{g_i(y_{i,l}^t)}^2}\\
	& \le \eta_l^2 K^2 \sum_{k =0}^{K-1} \E{\norm{g_i(y_{i, k}^t)}^2}\\
%	& \le K \eta_l^2 \sum_{k=0}^{K-1}\sum_{l=0}^{K-1} \E{\norm{g_i(y_{i,l}^t)}^2}\\
	& = \eta_l^2 K^2 \sum_{k=0}^{K-1} \left[ \E{\norm{g_i(y_{i,l}^t) - \nabla \Lcal_i(y_{i,l}^t)}^2}+ \E{\norm{\nabla \Lcal_i(y_{i,l}^t)}^2}\right]\\
	& \stackrel{A\ref{ass:unbiased}}{\le} \eta_l^2 K^3 \sigma^2 + \eta_l^2 K^2 \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i, k}^t)}^2}\label{app:eq:B_5}\\ 
	& \stackrel{(\ref{app:eq:B_2})}{\le} \eta_l^2 K^3 \sigma^2 
	+ 2 \eta_l^2 K^2 L^2 \sum_{k=0}^{K-1} \E{\norm{y_{i, k}^t - \theta^t}^2}
	+ 2 \eta_l^2 K^3\E{\norm{\nabla \Lcal_i(\theta^t)}^2}  ,
	\end{align}	

	We consider $\eta_l \le \frac{1}{2 L K}$ which implies that $ 1 - 2 \eta_l^2 L^2 K^2 \ge 1/2$ giving
	\begin{equation}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	\le 2 \eta_l^2 K^3[\sigma^2 + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}].
	\label{app:eq:B_4}
	\end{equation}
	
	Considering $\eta_l \le \frac{1}{2 L K}$ and substituting equation (\ref{app:eq:B_4}) in equation (\ref{app:eq:B_3}) completes the proof.
\end{proof}




%\begin{lemma}\label{lem:bounded_drift}
%	Under Assumptions \ref{ass:smoothness} and \ref{ass:unbiased} and for a local learning rate satisfying $\eta_l \le 1/2 L K$, a client drift can be bounded as
%	\begin{equation}
%%	\E{\norm{y_{i,k}^t - \theta^t}^2} \le
%	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
%	\le 4 \eta_l^2 K^3 \E{\norm{\nabla \Lcal_i(\theta^t)}^2} + 2 \eta_l^2 K^3\sigma^2.
%	\end{equation}
%\end{lemma}
%
%\begin{proof}	
%	By construction, we have $y_{i,k}^t - \theta^t = - \sum_{l=0}^{k-1} \eta_l g_i(y_{i,l}^t)$. Using Jensen's inequality, we get:
%	\begin{align}
%	\E{\norm{y_{i,k}^t - \theta^t}^2}
%	& \le k \sum_{l=0}^{k-1} \eta_l^2\E{\norm{g_i(y_{i,l}^t)}^2}\\
%	& \le K \eta_l^2 \sum_{l=0}^{K-1} \E{\norm{g_i(y_{i,l}^t)}^2}\\
%	& = K \eta_l^2 \sum_{l=0}^{K-1} \left[ \E{\norm{g_i(y_{i,l}^t) - \nabla \Lcal_i(y_{i,l}^t)}^2}+ \E{\norm{\nabla \Lcal_i(y_{i,l}^t)}^2}\right]\\
%	& \le \eta_l^2 K^2 \sigma^2 + \eta_l^2 K \sum_{k=0}^{K-1} \E{\norm{\nabla \Lcal_i(y_{i,l}^t)}^2},\label{app:eq:B_1}
%	\end{align}
%	where the equality comes from the unbiasedness of the SGD estimator, Assumption \ref{ass:unbiased}, and the last inequality comes from the bounded variance of the SGD estimator, Assumption \ref{ass:unbiased}.
%
%	In addition, we can bound a gradient descent as:
%	\begin{align}
%	\E{\norm{\nabla \Lcal_i(y_{i,k}^t)}^2}
%	& \le 2 \E{\norm{\nabla \Lcal_i(y_{i,k}^t) - \nabla \Lcal_i(\theta^t)}^2} + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}\\
%	& \le 2 L^2 \E{\norm{y_{i,k}^t - \theta^t}^2} + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}\label{app:eq:B_2}
%	\end{align}
%	Substituting equation (\ref{app:eq:B_2}) in equation (\ref{app:eq:B_1}), we get:
%	\begin{align}
%	\E{\norm{y_{i,k}^t - \theta^t}^2}
%	& \le \eta_l^2 K^2 \sigma^2 + 2 \eta_l^2 K L^2 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2} + 2 \eta_l^2 K^2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}\label{app:eq:B_3}
%	\end{align}
%	Summing over $k$ with equation (\ref{app:eq:B_3}), we get:
%	\begin{align}
%	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
%	& \le \eta_l^2 K^3 \sigma^2 + 2 \eta_l^2 L^2 K^2 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2} + 2 \eta_l^2 K^3E{\norm{\nabla \Lcal_i(\theta^t)}^2}
%	\end{align}
%	We consider $\eta_l \le \frac{1}{2 L K}$ which completes the proof:
%	\begin{equation}
%%	\E{\norm{y_{i,k}^t - \theta^t}^2} \le
%	 \sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
%	 \le 2 \eta_l^2 K^3[\sigma^2 + 2 \E{\norm{\nabla \Lcal_i(\theta^t)}^2}]
%	\end{equation}
%\end{proof}





\subsubsection{Proof of Theorem \ref{theo:convergence_dissimilarity}}\label{app:proof:convergence}

\begin{theorem}[FL convergence with Assumption \ref{ass:dissimilarity}]\label{theo:convergence_dissimilarity}
	Under Assumptions \ref{ass:smoothness} to \ref{ass:dissimilarity}, with convex local loss functions, with small enough local step size $\eta_l = \sqrt{m/KT}$, and with a client sampling satisfying Definition \ref{def:sampling} and with $\VAR{\omega_i(S_t)} = a_1 p_i^2 + a_2 p_i$, and with $\COV{\omega_j(S_t)}{\omega_k(S_t)} = -\alpha p_i p_j$, we get the following convergence bound:
	\begin{align}
	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
	& \le \Ocal(\frac{1}{\eta_g \eta_l T})+ \Ocal(\eta_l^2K^2) +\Ocal (\eta_g \eta_l K \delta^*),
	\end{align}
	where 
	\begin{equation}
	\delta^*
	=
	\left[\max\{(a_1 + \alpha ) p_{min}, (a_1 + \alpha ) p_{max}\}  + a_2 + (1- \mu^*) (1 - \alpha) \right]
	\ge 
	\delta.
	\end{equation}
\end{theorem}


\begin{proof}
	
	By substituting $\EE{t}{\theta_i^{t+1} - \theta^t} = \sum_{k=0}^{K-1} \EE{t}{\nabla \Lcal(y_{i, k}^t)}$ in equation (\ref{eq:one_server_iteration_bound}), we get:
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	\underbrace{- 2 \tilde{\eta} \inner{\sum_{k, i}p_i \EE{t}{\nabla \Lcal_i(y_{i,k}^t)} }{\theta^t - \theta^*}}_{T_1} + \underbrace{\eta_g^2 \sum_{i=1}^{n}\delta_i \EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 }}_{T_2},  \label{app:eq:C_1}
	\end{align}
%	with 
%%	\begin{equation}
%%	\delta_i^t 
%%	= \VARR{S_t}{\omega_i(S_t)} - \alpha p_i^2 + (1 - \gamma^t)(1+ \alpha) p_i .
%%	\end{equation}
%	\begin{equation}
%	\delta_i
%	= \VARR{S_t}{\omega_i(S_t)} - \alpha p_i^2 + (1+ \alpha) p_i .
%	\end{equation}
	
	
	
	\subsubsection*{Bounding $T_1$}
	Using Lemma \ref{lem:perturbed_strong_convexity} with convex functions ($\mu = 0$), we can bound $T_1$ as :
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} \sum_{k, i}p_i \left[ \Lcal_i(\theta^t) - \Lcal_i(\theta^*) - L \EE{t}{\norm{y_{i, k}^t - \theta^t}^2}
	%		+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right]\\
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
	%		+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] + 2 L \tilde{\eta} \sum_{i}p_i\sum_{k}\EE{t}{\norm{y_{i,k}^t - \theta^t}^2},
	\end{align}
	where $\sum_{k} \EE{t}{\norm{y_{i,k}^t - \theta^t}^2}$ can be bounded using Lemma \ref{lem:bounded_drift}:
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} K\left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] + 4L \tilde{\eta} \eta_l^2 K^3 \left[2 \sum_{i=1}^{n}p_i\norm{\nabla \Lcal_i(\theta^t)}^2 + \sigma^2 \right] \\
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] + 4L \tilde{\eta} \eta_l^2 K^3 \left[2 \beta^2 \norm{\nabla \Lcal(\theta^t)}^2 + \sigma^2 + 2 \kappa^2\right], \label{app:eq:C_2}
	\end{align}
	where the last inequality comes from using Assumption \ref{ass:dissimilarity}.
	
	
	
	
	\subsubsection*{Bounding $\delta_i$}
	Using the assumption on the expression of every client's stochastic weight, we get:
	\begin{align}
	\delta_i
	&= \VARR{S_t}{\omega_i(S_t)} + \alpha p_i^2 + ( 1 - \mu^*) (1 - \alpha) p_i \\
	&= \left[a_1 + \alpha \right]p_i^2 + \left[a_2 + ( 1- \mu^*)(1+ \alpha) \right]p_i 
	\end{align}
	We do not make any assumption on the sign of $a_1 - \alpha$. Hence, we have:
	\begin{align}
	a_1 - \alpha \le 0 
	& \Rightarrow
	\delta_i^t 
	\le \left[(a_1 - \alpha ) p_{min} + a_2 + ( 1- \mu^*)(1+ \alpha)\right]p_i \\
	a_1 - \alpha \ge 0 
	& \Rightarrow
	\delta_i^t 
	\le \left[(a_1 - \alpha ) p_{max} + a_2 + ( 1- \mu^*)(1+ \alpha) \right]p_i 
	\end{align}
	which gives:
	\begin{equation}
	\delta_i
	\le 
	\underbrace{\left[\max\{(a_1 - \alpha ) p_{min}, (a_1 - \alpha ) p_{max}\}  + a_2 + ( 1- \mu^*)(1+ \alpha) \right]}_{\delta^*} p_i \label{app:eq:C_3}
	\end{equation}
	
	We note that 
	\begin{equation}
		\delta^* 
		\ge\sum_{i =1 }^n \left[\left[a_1 - \alpha \right]p_i^2 + \left[a_2 + ( 1- \mu^*)(1+ \alpha) \right]p_i \right]
		= \delta 
	\end{equation}
	
	
	
	\subsubsection*{Bounding $T_2$}	
	Using equation (\ref{app:eq:C_3}), we can rewrite $T_2$ as :
	\begin{align}
	T_2
	\le 
	\eta_g^2 \delta^* \sum_{i=1}^{n} p_i\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 }
	\end{align}
	
	We can also use Lemma \ref{lem:bounded_drift} to bound $\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 } $ which gives :
	\begin{align}
	T_2
	\le 2 K^2 \tilde{\eta}^2 \delta^* \left[2 \sum_{i =1 }^n p_i \norm{\nabla \Lcal_i(\theta^t)}^2 + \sigma^2 \right]\\
	\le 2 K^2 \tilde{\eta}^2 \delta^* \left[ 2 \beta^2 \norm{\nabla \Lcal(\theta^t)}^2 + 2 \kappa^2 + \sigma^2 \right], \label{app:eq:C_4}
	\end{align}
	where the last inequality comes from using Assumption \ref{ass:dissimilarity}.
	
	
	
	
	\subsubsection*{Bounding equation (\ref{app:eq:C_1})}
	Substituting equation (\ref{app:eq:C_4}) and (\ref{app:eq:C_2}) in equation (\ref{app:eq:C_1}), we get:	
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
	\right] \nonumber\\
	&+ 4L \tilde{\eta} \eta_l^2 K^3 \left[2 \beta^2 \norm{\nabla \Lcal(\theta^t)}^2 + \sigma^2 + 2 \kappa^2 \right]\nonumber\\
	&+ 2 K^2 \tilde{\eta}^2 \delta^* \left[2 \beta^2 \norm{\nabla \Lcal(\theta^t)}^2 + \sigma^2 + 2 \kappa^2 \right]  \\
	%	
	&= \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
	\right] \nonumber\\
	&+ 2 K^2 \tilde{\eta} \left[ 2L \eta_l^2 K+  \tilde{\eta} \delta^* \right] \left[2 \beta^2 \norm{\nabla \Lcal(\theta^t)}^2 + \sigma^2 + 2 \kappa^2 \right]  
	\end{align}
	The local loss functions are $L$-smooth, Assumption \ref{ass:smoothness}. Thus $\Lcal$ is also $L$-smooth and $\norm{\nabla \Lcal(\theta^t)}^2 \le 2 L (\Lcal(\theta^t) - \Lcal^*)$ which leads to
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 	
	&\le \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} K \left[ 1 - 4 L K \beta^2 \left[ 2L \eta_l^2 K +  \tilde{\eta} \delta^* \right] \right] \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
	\right] \nonumber\\
	&+ 2 K^2 \tilde{\eta} \left[ 2L \eta_l^2 K +  \tilde{\eta} \delta^* \right] \left[\sigma^2 + 2 \kappa^2 \right] \\ 
	&\le \norm{\theta^t - \theta^*}^2 
	- \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right]
	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
	+ 2 K^3 \tilde{\eta} \left[ 2L \eta_l^2 +  \tilde{\eta} \delta^* \right] \left[\sigma^2 + 2 \kappa^2 \right] 
	\end{align}
	where the last inequality comes from considering that $1 - 4 L K \beta^2 [ 2L \eta_l^2 K +  \tilde{\eta} \delta^*] \ge 1/2$.
	
	Finally, by rearranging the terms, we get:
	\begin{align}
	\E{\Lcal(\theta^t)} - \Lcal(\theta^*) 	
	& \le \frac{1}{\tilde{\eta} K} \left[\E{\norm{\theta^t - \theta^*}^2} - \E{\norm{\theta^{t+1} - \theta^*}^2}  \right] \nonumber\\
	&+ 2 K \left[ 2L \eta_l^2 K +  \tilde{\eta} \delta^* \right] \left[\sigma^2 + 2 \kappa^2 \right],
	\end{align}
	which gives:
	\begin{align}
	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
	& \le \frac{1}{\tilde{\eta} K (T+1)} \E{\norm{\theta^{0} - \theta^*}^2}  \nonumber\\
	&+ 2 K \left[ 2L \eta_l^2 K +  \tilde{\eta} \delta^*\right] \left[\sigma^2 + 2 \kappa^2 \right]\\
	& \le \Ocal(\frac{1}{\tilde{\eta} K T})+ \Ocal(K^2 \eta_l^2) +\Ocal (K  \tilde{\eta} \delta^*)
	\end{align}
	
% 	Finally, considering $\eta_l = \sqrt{m/KT}$  gives the following convergence guarantees:
% 	\begin{align}
% 	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
% 	& \le \Ocal(\frac{1}{\eta_g \sqrt{m K T}})+ \Ocal(\frac{mK}{T}) +\Ocal (\sqrt{\frac{{mK}}{{T}}} \eta_g\delta^*),
% 	\end{align}
% 	and shows that the global model converges to its optimum at infinity.
	
	
\end{proof}




%\subsection{Proof of Theorem \ref{theo:convergence}}\label{app:proof:convergence}
%
%\begin{proof}
%
%	With Lemma \ref{lem:equality_update_without_Jenken}, we get:
%	\begin{align}
%	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
%	&\le \norm{\theta^t - \theta^*}^2 
%	\underbrace{- 2 \tilde{\eta} \inner{\sum_{k, i}p_i \nabla \Lcal_i(y_{i,k}^t)}{\theta^t - \theta^*}}_{T_1} + \underbrace{\eta_g^2 \sum_{i=1}^{n}\delta_i^t\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 }}_{T_2},  \label{app:eq:C_1}
%	\end{align}
%%	with $A^t = \sum_{i=1}^n\left[\VARR{S_t}{\omega_i(S_t)} - \alpha p_i^2 + (1+ \alpha) p_i - \gamma^t (1+\alpha) p_i\right]$. 
%	with 
%	\begin{equation}
%		\delta_i^t 
%		= \VARR{S_t}{\omega_i(S_t)} - \alpha p_i^2 + (1 - \gamma^t)(1+ \alpha) p_i .
%	\end{equation}
%	
%	
%	
%	\subsubsection{Bounding $T_1$}
%	Using Lemma \ref{lem:perturbed_strong_convexity} with convex functions ($\mu = 0$), we can bound $T_1$ as :
%	\begin{align}
%	T_1 
%	&\le - 2 \tilde{\eta} \sum_{k, i}p_i \left[ \Lcal(\theta^t) - \Lcal(\theta^*) - L \norm{y_{i, k}^t - \theta^t}^2
%	%		+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
%	\right]\\
%	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
%	%		+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
%	\right] + 2 L \tilde{\eta} \sum_{i}p_i\sum_{k}\EE{t}{\norm{y_{i,k}^t - \theta^t}^2},
%	\end{align}
%	where $\sum_{k}p_i\EE{t}{\norm{y_{i,k}^t - \theta^t}^2}$ can be bounded using Lemma \ref{lem:bounded_drift}:
%	\begin{align}
%	T_1 
%	&\le - 2 \tilde{\eta} K\left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
%	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
%	\right] + 4L \tilde{\eta} \eta_l^2 K^3 \left[2 \sum_{i=1}^{n}p_i\E{\norm{\nabla \Lcal_i(\theta^t)}^2} + \sigma^2 \right] \\
%	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
%	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
%	\right] + 4L \tilde{\eta} \eta_l^2 K^3 \left[2 \beta^2 \E{\norm{\nabla \Lcal(\theta^t)}^2} + \sigma^2 + 2 \kappa^2\right], \label{app:eq:C_2}
%	\end{align}
%	where the last inequality comes from using Assumption \ref{ass:dissimilarity}.
%	
%	
%	
%	
%	\subsubsection{Bounding $\delta_i^t$}
%	We first start by bounding $\delta_i^t$ using the assumption on the expression of every client's stochastic weight:	
%	\begin{align}
%	\delta_i^t 
%	&= \VARR{S_t}{\omega_i(S_t)} - \alpha p_i^2 + (1 - \gamma^t)(1+ \alpha) p_i \\
%	&= \left[a_1 - \alpha \right]p_i^2 + \left[a_2 + (1 - \gamma^t)(1+ \alpha) \right]p_i 
%	\end{align}
%	We do not make any assumption on the sign of $a_1 - \alpha$. Hence, we have:
%	\begin{align}
%	a_1 - \alpha \le 0 
%	& \Rightarrow
%	\delta_i^t 
%	\le \left[(a_1 - \alpha ) p_{min} + a_2 + (1 - \gamma^t)(1+ \alpha) \right]p_i \\
%	a_1 - \alpha \ge 0 
%	& \Rightarrow
%	\delta_i^t 
%	\le \left[(a_1 - \alpha ) p_{max} + a_2 + (1 - \gamma^t)(1+ \alpha) \right]p_i 
%	\end{align}
%	which gives:
%	\begin{equation}
%	\delta_i^t 
%	\le \left[\max\{(a_1 - \alpha ) p_{min}, (a_1 - \alpha ) p_{max}\}  + a_2 + (1 - \gamma^t)(1+ \alpha) \right]p_i 
%	= \delta^* p_i \label{app:eq:C_3}
%	\end{equation}
%	
%	WE NEED TO PROVE THAT $\delta$ IS NON NEGATIVE.
%	
%	
%	
%	\subsubsection{Bounding $T_2$}	
%	Using equation (\ref{app:eq:C_3}), we can rewrite $T_2$ as :
%	\begin{align}
%	T_2
%	\le 
%	\eta_g^2 \delta^* \sum_{i=1}^{n} p_i\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 }
%	\end{align}
%		
%	We can also use Lemma \ref{lem:bounded_drift} to bound $\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 } $ which gives :
%	\begin{align}
%	T_2
%	\le 2 K^3 \tilde{\eta}^2 \delta^* \left[2 \sum_{i =1 }^n p_i \E{\norm{\nabla \Lcal_i(\theta^t)}^2} + \sigma^2 \right]\\
%	\le 2 K^3 \tilde{\eta}^2 \delta^* \left[ 2 \beta^2 \E{\norm{\nabla \Lcal(\theta^t)}^2} + 2 \kappa^2 + \sigma^2 \right], \label{app:eq:C_4}
%	\end{align}
%	where the last inequality comes from using Assumption \ref{ass:dissimilarity}.
%	
%	
%	
%	
%	\subsubsection{Bounding equation (\ref{app:eq:C_1})}
%	Substituting equation (\ref{app:eq:C_4}) and (\ref{app:eq:C_2}) in equation (\ref{app:eq:C_1}), we get:	
%	\begin{align}
%	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
%	&\le \norm{\theta^t - \theta^*}^2 
%	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
%%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
%	\right] \nonumber\\
%	&+ 4L \tilde{\eta} \eta_l^2 K^3 \left[2 \beta^2 \E{\norm{\nabla \Lcal(\theta^t)}^2} + \sigma^2 + 2 \kappa^2 \right]\nonumber\\
%	&+ 2 K^3 \tilde{\eta}^2 \delta\left[2 \beta^2 \E{\norm{\nabla \Lcal(\theta^t)}^2} + \sigma^2 + 2 \kappa^2 \right]  \\
%%	
%	&= \norm{\theta^t - \theta^*}^2 
%	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
%	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
%	\right] \nonumber\\
%	&+ 2 K^3 \tilde{\eta} \left[ 2L \eta_l^2 +  \tilde{\eta} \delta^* \right] \left[2 \beta^2 \E{\norm{\nabla \Lcal(\theta^t)}^2} + \sigma^2 + 2 \kappa^2 \right]  
%	\end{align}
%	The local loss functions are $L$-smooth, Assumption \ref{ass:smoothness}. Thus $\Lcal$ is also $L$-smooth and $\norm{\nabla \Lcal(\theta^t)}^2 \le 2 L (\Lcal(\theta^t) - \Lcal^*)$ which leads to
%	\begin{align}
%	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 	
%	&\le \norm{\theta^t - \theta^*}^2 
%	- \left[2 \tilde{\eta} K - 8 L K^3 \beta^2 \tilde{\eta} \left[ 2L \eta_l^2 +  \tilde{\eta} \delta^* \right] \right] \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
%	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
%	\right] \nonumber\\
%	&+ 2 K^3 \tilde{\eta} \left[ 2L \eta_l^2 +  \tilde{\eta} \delta^* \right] \left[\sigma^2 + 2 \kappa^2 \right] \\ 
%	&\le \norm{\theta^t - \theta^*}^2 
%	- \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) \right]
%	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
%	+ 2 K^3 \tilde{\eta} \left[ 2L \eta_l^2 +  \tilde{\eta} \delta^* \right] \left[\sigma^2 + 2 \kappa^2 \right] 
%	\end{align}
%	where the last inequality comes from considering that $8 L K^2 \beta^2 \left[ 2L \eta_l^2 +  \tilde{\eta} \delta^* \right] \le 1$.
%	
%	Finally, by rearranging the terms, we get:
%	\begin{align}
%	\E{\Lcal(\theta^t)} - \Lcal(\theta^*) 	
%	& \le \frac{1}{\tilde{\eta} K} \left[\E{\norm{\theta^t - \theta^*}^2} - \E{\norm{\theta^{t+1} - \theta^*}^2}  \right] \nonumber\\
%	&+ 2 K^2 \left[ 2L \eta_l^2 +  \tilde{\eta} \delta^* \right] \left[\sigma^2 + 2 \kappa^2 \right],
%	\end{align}
%	which gives:
%	\begin{align}
%	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
%	& \le \frac{1}{\tilde{\eta} K (T+1)} \E{\norm{\theta^{0} - \theta^*}^2}  \nonumber\\
%	&+ 2 K^2 \left[ 2L \eta_l^2 +  \tilde{\eta} \frac{1}{T+1}\sum_{t=0}^{T}\delta^*\right] \left[\sigma^2 + 2 \kappa^2 \right]\\
%	& \le \Ocal(\frac{1}{\tilde{\eta} K T})+ \Ocal(K^2 \eta_l^2) +\Ocal (K^2  \tilde{\eta} \frac{1}{T}\sum_{t=0}^{T}\delta^*)
%	\end{align}
%
%	We consider $\gamma^*$ the minimum Jensen gap such that $\gamma^t \ge \gamma^* > 0$. Hence, there is a $\delta^*$ such that $1 < \delta^* \le \delta^* $ which gives:
%	\begin{align}
%	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
%	& \le \Ocal(\frac{1}{\tilde{\eta} KT})+ \Ocal(K^2 \eta_l^2) +\Ocal (K^2  \tilde{\eta} \delta^*)
%	\end{align}
%	
%	Finally, considering $\eta_l = \sqrt{m/KT}$  gives the following convergence guarantees:
%	\begin{align}
%	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
%	& \le \Ocal(\frac{1}{\eta_g \sqrt{m K T}})+ \Ocal(\frac{mK}{T}) +\Ocal (\frac{m K \sqrt{K} \eta_g}{\sqrt{T}}\delta^*),
%	\end{align}
%	and shows that the global model converges to its optimum at infinity.
%	
%	
%\end{proof}














% \begin{corollary}[FL convergence with Assumption \ref{ass:bounded_gradient}]\label{cor:convergence_bounded}
% 	When considering Assumption \ref{ass:bounded_gradient} instead of Assumption \ref{ass:dissimilarity}, and without requiring $\VAR{\omega_i(S_t)} = a_1 p_i^2 + a_2 p_i$, the convergence bound of Theorem \ref{theo:convergence} still holds for :
% 	\begin{equation}
% 	\delta^*
% 	=
% 	\sum_{i=1}^{n}\gamma_i + (1- \mu^*) (1 - \alpha) 
% 	= \delta - \mu^* (1 - \alpha) 
% 	\end{equation}
% \end{corollary}

% We provide the proof for Corollary \ref{cor:convergence_bounded} in Appendix XX. We note that by assuming that the local loss functions are strongly convex, identical convergence to Corollary \ref{cor:convergence_bounded} can be proven without Assumption \ref{ass:dissimilarity} or \ref{ass:bounded_gradient} and can be found in Theorem \ref{theo:convergence_2} with proof in Appendix \ref{app:proof:convergence_2}. Consistently with Theorem \ref{theo:convergence} and the rest of FL literature, FL asymptotically converge to its optimum and any unbiased clients sampling provides identical convergence rate. 

% We also note that in the special case, where all the clients have the same data distribution, we have $\mu^*=0$ which gives $\delta^* = \delta$. Hence, even if all the clients have the same data distribution, a slow-down is incurred by the sum of the aggregation weight variance.
	
	
\subsection{FL convergence guarantees with Assumption \ref{ass:bounded_gradient}}\label{app:sec:convergence_ass_4}


\subsubsection{Bounding the client drift}
\begin{lemma}\label{lem:bounded_drift_ass_bounded}
	Under Assumption \ref{ass:smoothness} and \ref{ass:unbiased}, a client drift can be bounded as
	\begin{equation}
	\E{\norm{\theta_i^{t+1} - \theta^t}^2} 
	\le \eta_l^2 K^2[\sigma^2 + G^2], 
	\end{equation}
	and 
	\begin{equation}
	\sum_{k=0}^{K-1} \E{\norm{y_{i,k}^t - \theta^t}^2}
	\le \eta_l^2 K^3[\sigma^2 + G^2].
	\end{equation}
\end{lemma}

\begin{proof}	
    By using Assumption \ref{ass:bounded_gradient} in equation (\ref{app:eq:B_1}) and (\ref{app:eq:B_5}), the proof follows directly.
\end{proof}






\subsubsection{Proof of Theorem \ref{theo:convergence_bounded}}\label{app:proof:convergence_bounded_grad}

\begin{theorem}[FL convergence with Assumption \ref{ass:bounded_gradient}]\label{theo:convergence_bounded}
	Under Assumptions \ref{ass:smoothness} to \ref{ass:dissimilarity}, with convex local loss functions, with small enough local step size, and with a client sampling satisfying Definition \ref{def:sampling} and with $\VAR{\omega_i(S_t)} = a_1 p_i^2 + a_2 p_i$, and with $\COV{\omega_j(S_t)}{\omega_k(S_t)} = -\alpha p_i p_j$, we get the following convergence bound:
	\begin{align}
	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
	& \le \Ocal(\frac{1}{\tilde{\eta} K T})+ \Ocal(K^2 \eta_l^2) +\Ocal (K  \tilde{\eta} \delta).
	\end{align}

\end{theorem}


\begin{proof}
	
	By substituting $\EE{t}{\theta_i^{t+1} - \theta^t} = \sum_{k=0}^{K-1} \EE{t}{\nabla \Lcal(y_{i, k}^t)}$ in equation (\ref{eq:one_server_iteration_bound}), we get:
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	\underbrace{- 2 \tilde{\eta} \inner{\sum_{k, i}p_i \EE{t}{\nabla \Lcal_i(y_{i,k}^t)} }{\theta^t - \theta^*}}_{T_1} + \underbrace{\eta_g^2 \sum_{i=1}^{n}\delta_i \EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 }}_{T_2},  \label{app:eq:U_1}
	\end{align}
	
	\subsubsection*{Bounding $T_1$}
	Using Lemma \ref{lem:perturbed_strong_convexity} with convex functions ($\mu = 0$), we can bound $T_1$ as :
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} \sum_{k, i}p_i \left[ \Lcal_i(\theta^t) - \Lcal_i(\theta^*) - L \EE{t}{\norm{y_{i, k}^t - \theta^t}^2}
% 			+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right]\\
	&\le - 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
			+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] + 2 L \tilde{\eta} \sum_{i}p_i\sum_{k}\EE{t}{\norm{y_{i,k}^t - \theta^t}^2},
	\end{align}
	where $\sum_{k} \EE{t}{\norm{y_{i,k}^t - \theta^t}^2}$ can be bounded using Lemma \ref{lem:bounded_drift_ass_bounded}:
	\begin{align}
	T_1 
	&\le - 2 \tilde{\eta} K\left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
% 		+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2
	\right] 
	+ 2L \tilde{\eta} \eta_l^2 K^3 \left[\sigma^2 + G^2 \right].  \label{app:eq:U_2}
	\end{align}
	

	
	
	\subsubsection*{Bounding $T_2$}	
	We can use Lemma \ref{lem:bounded_drift_ass_bounded} to bound $\EE{t}{\norm{\theta_i^{t+1} - \theta^t}^2 } $ in $T_2$ which gives :
	\begin{align}
	T_2
	\le \tilde{\eta}^2 K^2 [\sigma^2 + G^2]\delta. \label{app:eq:U_4}
	\end{align}
	
	
	
	
	\subsubsection*{Bounding equation (\ref{app:eq:C_1})}
	Substituting equation (\ref{app:eq:U_4}) and (\ref{app:eq:U_2}) in equation (\ref{app:eq:U_1}), we get:	
	\begin{align}
	\EE{t}{\norm{\theta^{t+1} - \theta^*}^2} 
	&\le \norm{\theta^t - \theta^*}^2 
	- 2 \tilde{\eta} K \left[ \Lcal(\theta^t) - \Lcal(\theta^*) 
	%	+ \frac{\mu}{4}\norm{\theta^t - \theta^*}^2 
	\right] \nonumber\\
	&+ 2L \tilde{\eta} \eta_l^2 K^3 \left[\sigma^2 + G^2 \right] 
	+ \tilde{\eta}^2 K^2 [\sigma^2 + G^2]\delta  
	\end{align}
	
	By rearranging the terms, we get:
	\begin{align}
	\E{\Lcal(\theta^t)} - \Lcal(\theta^*) 	
	& \le \frac{1}{2\tilde{\eta} K} \left[\E{\norm{\theta^t - \theta^*}^2} - \E{\norm{\theta^{t+1} - \theta^*}^2}  \right] \nonumber\\
	&+ L \eta_l^2 K^2 \left[\sigma^2 + G^2 \right] 
	+ \frac{1}{2}\tilde{\eta} K [\sigma^2 + G^2]\delta  ,
	\end{align}
	which gives:
	\begin{align}
	\frac{1}{T+1} \sum_{t=0}^{T}\left[\E{\Lcal(\theta^t)} - \Lcal(\theta^*) \right]	
	& \le \frac{1}{2 \tilde{\eta} K (T+1)} \E{\norm{\theta^{0} - \theta^*}^2}  \nonumber\\
	&+ L \eta_l^2 K^2 \left[\sigma^2 + G^2 \right] 
	+ \frac{1}{2}\tilde{\eta} K [\sigma^2 + G^2]\delta\\
	& = \Ocal(\frac{1}{\tilde{\eta} K T})+ \Ocal(K^2 \eta_l^2) +\Ocal (K  \tilde{\eta} \delta)
	\end{align}
	
\end{proof}


==> tex/properties.tex <==

\section{Properties}\label{app:sec:properties}

We have: 
\begin{equation}
	\COV{\omega_i(S_t)}{\omega_j(S_t)}
	= \E{\omega_i(S_t)\omega_j(S_t)} - p_i p_j
	\ge - p_i p_j
\end{equation}
Hence, we have $\alpha \ge 1 $. 

We also have:
\begin{align}
	\VAR{\sum_{i=1}^{n}\omega_i(S_t)}
	&= \sum_{i=1}^{n}\VAR{\omega_i(S_t)}
	+ \sum_{i, j\neq i} \COV{\omega_i(S_t)}{\omega_j(S_t)}\\
	&= \sum_{i=1}^{n}\VAR{\omega_i(S_t)}
	- \alpha \sum_{i, j\neq i} p_i p_j\\
	&= \sum_{i=1}^{n}\left[ \VAR{\omega_i(S_t)}- \alpha p_i (1 - p_i)\right] \label{app:eq:U_1}\\
	&= \sum_{i=1}^{n}\gamma_i - \alpha 
\end{align}

Let us assume that there exists a function $f$ such that $\VAR{\omega_i(S_t)} = f ( p_i) \ge 0$ and $\sum_{i=1}^{n}\omega_i(S_t) = 1$. Using equation (\ref{app:eq:U_1}), we get:
\begin{align}
	\sum_{i=1}^{n}\left[ f(p_i)- \alpha p_i (1 - p_i)\right] = 0
\end{align}

$\alpha<0 \Rightarrow f(p_i) - \alpha p_i(1 - p_i) > 0$ which is not possible. Hence $\alpha \ge 0$. 

If we suppose in addition that $f(p_i) = a_1 p_i^2 + a_2 p_i$, we get:
\begin{align}
	(a_1 + \alpha)\sum_{i=1}^{n} p_i^2 +(a_2 - \alpha) = 0 
	& \Rightarrow a_1 = -\alpha \text{ and } a_2 = \alpha \\
	& \Rightarrow \VAR{\omega_i(S_t)} = \alpha p_i ( 1 - p_i) \\
	& \Rightarrow \gamma_i = \alpha p_i
\end{align}
 
 
 \newpage

==> tex/quadratic.tex <==
\newpage
\section{Quadratic}\label{app:sec:quadratic}


\begin{proof}
	For every client, we consider local loss functions such that:
	\begin{equation}
		\Lcal_i(\vtheta)
		= \frac{1}{2}\norm{\vtheta - \vtheta_i^*}^2,
	\end{equation}
	where $\vtheta_i^*$ is client's $i$ local minimum. By taking the derivative of the global loss function, equation (\ref{eq:global_loss}), with these clients local loss function, gives:
	\begin{equation}
		\vtheta^* 
		= \sum_{i =1}^n p_i \vtheta_i^*.
	\end{equation} 
	
	$\vy_{i, k}^t$ is the local model obtained for client $i$ after $k$ SGD and satisfies 
	\begin{equation}
		\vy_{i, k+1}^t 
		= \vy_{i, k}^t - \eta_l (\vy_{i, k}^t - \vtheta_i^*)
		= (1 - \eta_l) \vy_{i, k}^t + \eta_l \vtheta_i^*, 
	\end{equation}
	which, by induction, gives
	\begin{equation}
	\vtheta_i^{t+1} 
	= (1 - \eta_l)^K \vtheta^t + \sum_{k=0}^{K-1} ( 1 - \eta_l)^k \eta_l \vtheta_i^*. 
	\end{equation}
	We note that $\sum_{k=0}^{K-1} ( 1 - \eta_l)^k = [1 - ( 1 - \eta_l )^K]/ \eta_l$. By defining $\phi = 1 - ( 1 - \eta_l )^K$, we get:
	\begin{equation}
	\vtheta_i^{t+1} - \vtheta^t
	= (1 - \eta_l)^K \vtheta^t + \left[1 - ( 1 - \eta_l )^K \right] \vtheta_i^* - \vtheta^t
	= \phi (\vtheta_i^* - \vtheta^t). 
	\end{equation} 
	Hence, we have 
	\begin{equation}
		\sum_{i =1 }^n p_i (\vtheta_i^{t+1} - \vtheta^t)
		= \phi (\vtheta^* - \vtheta^t).
	\end{equation}
	Using Decomposition Property \ref{theo:decomposition_theorem} leads to
	\begin{align}
	\E{\norm{\vtheta^{t+1} - \vtheta^*}^2}
	& = 
	( 1- 2 \tilde{\eta})\E{\norm{\vtheta^{t} - \vtheta^*}^2} 
	+ \eta_g^2 \sum_{i=1}^{n}\gamma_i \phi^2 \E{\norm{\vtheta^t - \vtheta_i^*}^2}
	\nonumber\\
	&
	+ \eta_g^2 ( 1 - \alpha ) \phi^2 \E{\norm{\vtheta^t - \vtheta^*}^2}.
	\end{align}

\end{proof}



==> tex/sampling_properties.tex <==
\subsection{Clients' sampling properties}\label{app:sec:properties}

We have: 
\begin{equation}
	\COV{\omega_i(S_t)}{\omega_j(S_t)}
	= \E{\omega_i(S_t)\omega_j(S_t)} - p_i p_j
	\ge - p_i p_j
\end{equation}
Hence, we have $\alpha \ge 1 $. 

We also have:
\begin{align}
	\VAR{\sum_{i=1}^{n}\omega_i(S_t)}
	&= \sum_{i=1}^{n}\VAR{\omega_i(S_t)}
	+ \sum_{i, j\neq i} \COV{\omega_i(S_t)}{\omega_j(S_t)}\\
	&= \sum_{i=1}^{n}\VAR{\omega_i(S_t)}
	- \alpha \sum_{i, j\neq i} p_i p_j\\
	&= \sum_{i=1}^{n}\left[ \VAR{\omega_i(S_t)}- \alpha p_i (1 - p_i)\right] \label{app:eq:V_1}\\
	&= \sum_{i=1}^{n}\gamma_i - \alpha 
\end{align}

Let us assume that there exists a function $f$ such that $\VAR{\omega_i(S_t)} = f ( p_i) \ge 0$ and $\sum_{i=1}^{n}\omega_i(S_t) = 1$. Using equation (\ref{app:eq:V_1}), we get:
\begin{align}
	\sum_{i=1}^{n}\left[ f(p_i)- \alpha p_i (1 - p_i)\right] = 0
\end{align}

$\alpha<0 \Rightarrow f(p_i) - \alpha p_i(1 - p_i) > 0$ which is not possible. Hence $\alpha \ge 0$. 

If we suppose in addition that $f(p_i) = a_1 p_i^2 + a_2 p_i$, we get:
\begin{align}
	(a_1 + \alpha)\sum_{i=1}^{n} p_i^2 +(a_2 - \alpha) = 0 
	& \Rightarrow a_1 = -\alpha \text{ and } a_2 = \alpha \\
	& \Rightarrow \VAR{\omega_i(S_t)} = \alpha p_i ( 1 - p_i) \\
	& \Rightarrow \gamma_i = \alpha p_i
\end{align}

==> tex/sketch_proof.tex <==
\section{Sketch for Proof of Decomposition Theorem \ref{theo:decomposition_theorem} and Theorem \ref{theo:convergence_paper}}
